Toward a Complete Criterion for Value of Information in Insoluble Decision Problems

In a decision problem, observations are said to be material if they must be taken into account to perform optimally. Decision problems have an underlying (graphical) causal structure, which may sometimes be used to evaluate certain observations as immaterial. For soluble graphs - ones where important past observations are remembered - there is a complete graphical criterion; one that rules out materiality whenever this can be done on the basis of the graphical structure alone. In this work, we analyse a proposed criterion for insoluble graphs. In particular, we prove that some of the conditions used to prove immateriality are necessary; when they are not satisfied, materiality is possible. We discuss possible avenues and obstacles to proving necessity of the remaining conditions.

==> sections/old/n-analysing-thm2.tex <==
%\section{Further Thm 2}
%We would like to know, given an ordering graph $\calH$ for Le 1, for which there exists a 
%topological ordering, what further requirements on are placed (on $\prec$) by Thm 2?
%
%To address this question, I have begun by analysing a simpler question:
%given some $\calH$ and a topological ordering $\prec$, how do we know whether Thm 2
%is satisfied?
%
%\begin{lemma}
%If
%$\sZ \not \dsep (\sV' \setminus \fix(C_X \setminus \sZ ))_{\prec Z} \mid \fix(C_X \setminus \sZ )_{\prec Z}$
%then
%there exists a path $\sZ \ni Z \upathto V$ where $V \in (\sV' \setminus \fix(C_X \setminus \sZ ))_{\prec Z}$
%such that every collider is in $(\sC' \cap C_X)_{\prec Z}$
%and every non-collider is not in $\sV'$.
%\end{lemma}
%
%\begin{proof}
%By assumption, there exists some path 
%from $\sZ$ to $(\sV' \setminus \fix(C_X \setminus \sZ ))_{\prec Z}$, active given $\fix(C_X \setminus \sZ )_{\prec Z}$.
%Let $p:\sZ \ni Z \upathto V$ be the shortest such path.
%$p$ cannot contain any $(\sV' \setminus \fix(C_X \setminus \sZ ))_{\prec Z}$, except at $V$.
%
%We will prove that: 
%(1) $p \cap \sX' = \emptyset$,
%(2) $p$ does not contain any collider in $\sZ$,
%(3) $p$ does not contain any non-collider in $\sC'$
%(4) $p$ does not contain any non-collider in $\sZ$.
%We will use this to prove that $p$ satisfies the required conditions.
%
%Proof of 1) If $p$ contains a collider $X \in \sX'$, by activeness of $p$ given $\fix(C_X \setminus \sZ )_{\prec Z}$,
%$X \in \fix(C_X \setminus \sZ )_{\prec Z}$.
%Then, Le 1 implies that $\Pa^\calG_X \subseteq \sV'_{\prec Z}$.
%Moreover, $\Pa^\calG_X \subseteq \fix(C_X \setminus \sZ )_{\prec Z}$, since $X \in \fix(C_X \setminus \sZ )_{\prec Z}$.
%This would block $p$ and give a contradiction. So $p$ does not contain a collider $X \in \sX'$.
%If instead $p$ contains a non-collider $X \in \sX' \setminus \{V\}$, then 
%$X \not \in \sX' \cap \fix(C_X \setminus \sZ )_{\prec Z}$ by activeness of $p$, 
%and $X \not \in \sX' \setminus \fix(C_X \setminus \sZ )_{\prec Z}$, because it is not an endpoint.
%So $X \in \sX'_{\succ Z}$.
%We also know that $V \prec Z$. If $\sW$ denotes the set of colliders in $p$, then we also know 
%that $\sW \in \sV'_{\prec Z}$.
%It follows from Le 1 that $X \not \in \Anc^\calG_{Z \cup V \cup \sW}$.
%So $p$ cannot contain a non-collider $X \in \sX' \setminus \{C\}$.
%Thus $p$ cannot contain any $X \in \sX' \setminus \{V\}$.
%
%Proof of 2) Suppose $p$ contains a collider in $\sZ$, and we will prove a contradiction.
%Let $Z'$ be the collider $Z \in \sZ$ nearest to $V$ in $p$.
%By activeness of $p$, $Z' \in \fix(C_X \setminus \sZ )_{\prec Z}$.
%%We will prove that if $Z' \prec Z$, then $Z' \not \in \fix(C_X \setminus \sZ )$.
%Let $q:V \overset{p}{\upathto} Z'$.
%If $q$ is active given $\fix(C_X \setminus \sZ )_{\prec Z'}$, 
%then $Z' \not \in \fix(C_X \setminus \sZ )_{\prec Z}$, 
%\ryan{Not quite. This only applies if $V 
%\prec Z'$. We can also have $Z' 
%\in 
%\fix(C_X 
%\setminus 
%\sZ)_{\prec V}$.}
%giving a contradiction.
%So instead, suppose that $q$ is inactive given $\fix(C_X \setminus \sZ )_{\prec Z'}$. 
%%which will imply that $Z' \not \in \fix(C_X \setminus \sZ )$.
%We know $q$ does not contain any non-collider in $\fix(C_X \setminus \sZ )_{\prec Z'}$ by $q \subseteq p$ and $Z' \prec Z$.
%$q$ also is not blocked at any collider in $\sZ$ because $Z'$ was assumed to be the nearest collider in $\sZ$ to $V$. 
%Furthermore, $\fix(C_X \setminus \sZ )_{\prec Z} \cap p \cap \sX' = \emptyset$. 
%So $q$ must be blocked by a collider in $\sC'$.
%So let $C'$ be the nearest collider to $Z'$ in $q$ that is in $\sC' \setminus \fix(C_X \setminus \sZ )_{\prec Z'}$.
%Let $r:C' \overset{q}{\upathto} Z'$.
%From $r \subseteq p$, we know that $r$ does not contain any non-collider in $\fix(C_X \setminus \sZ )_{\prec Z}$ 
%(by activeness of $p$)
%nor any $\sV' \setminus \fix(C_X \setminus \sZ ))_{\prec Z}$ (because $p$ is a shortest path), 
%so $r$ cannot contain any non-collider in $\sV'_{\prec Z}$.
%$C'$ is a collider in $p$, so $C' \prec Z$, hence $r$ cannot contain any non-collider $\sV'_{\prec C'}$.
%$r$ also can't contain any collider in $\sZ$, since $Z'$ is the collider nearest $V$.
%Furthermore, we assumed that $C'$ is the collider nearest $Z'$ that is in $\sC' \setminus \fix(C_X \setminus \sZ )_{\prec Z'}$ (and $p$ cannot contain any $\fix(C_X \setminus \sZ )_{\prec Z'}$
%so every collider $C''$ in $r$ has $C'' \prec C'$.
%Thus $r:C' \upathto Z'$ is active given $\lceil(\sX' \cup \sC')_{\prec C}\rceil$.
%Hence by Le 1, we have $C' \prec Z'$, giving a contradiction.
%
%%Suppose that $r$ was blocked given $\lceil (\sX' \cup \sC')_{\prec C} \rceil$.
%%We have proved that this cannot be due to a non-collider, 
%%nor a collider $\sZ$, and $p$ does not contain any $\sX'$, 
%%so the only way this could occur is via a collider in $\sC'$.
%%But suppose so, and let $C''$ be the collider nearest $C'$ that blocked $r$.
%%Then, the path from $C''$ to $C'$ 
%%This collider must be in $\sC'$, because it must be in $\fix(C_X \setminus \sZ )$ but cannot be in $\sZ$ or $\sX'$.
%
%Proof of 3) %Now we prove that $p$ cannot contain a non-collider $C' \in \sC'$.
%Let $C'$ be the non-collider in $\sC'$ nearest to $Z$ in $p$, and we will prove a contradiction.
%Let $p':C' \overset{p}{\upathto} Z$.
%Let $Z'$ be the collider in $\sZ$ nearest to $C'$ in $p'$ and let $q:C' \overset{p'}{\upathto} Z'$.
%Since $p$ is the shortest path, it
%contains no $(\sV' \setminus \fix(C_X \setminus \sZ ))_{\prec Z}$.
%And by activeness of $p$, $C' \not \in \fix(C_X \setminus \sZ )_{\prec Z}$.
%So $Z \prec C'$.
%From activeness of $p$, every collider in $q$ is in $\sV'_{\prec Z}$.
%We have just proved that
%$p$ contains no collider in $\sX'$.
%Moreover, $q$ contains no collider in $\sZ$ by the definition of $Z'$.
%So every collider in $q$ is in $(\sC' \cap C_X)_{\prec Z}$,
%and hence in $(\sC' \cap C_X)_{\prec C'}$.
%By the definitions of $C'$ and $Z'$, $q$ contains no non-collider in $\sC' \cup Z'$, 
%and we have just proved that $p$ contains no non-collider $\sX'$.
%So $q$ is active given $\lceil(\sX' \cup \sC')_{\prec C} \rceil$.
%Hence $C' \prec Z'$ from Lemma 1.
%And $Z' \prec Z$, by the activeness of $p$.
%So $C' \prec Z'$.
%But this contradicts $Z \prec C'$.
%So $p$ cannot contain a non-collider in $\sC'$.
%
%%Let $C'$ be the non-collider in $\sC'$ nearest to $Z$ in $p$, and we will prove a contradiction.
%%Let $q:C' \overset{p}{\upathto} Z$.
%%Since $p$ is the shortest path, it
%%contains no $(\sV' \setminus \fix(C_X \setminus \sZ ))_{\prec Z}$.
%%And by activeness of $p$, $C' \not \in \fix(C_X \setminus \sZ )_{\prec Z}$.
%%So $Z \prec C'$.
%%From activeness of $p$, every collider in $q$ is in $\sV'_{\prec Z}$.
%%And we have just proved that
%%$p$ contains no collider in $\sX'$ or $\sZ$, 
%%So every collider in $q$ is in $(\sC' \cap C_X)_{\prec Z}$,
%%and hence in $(\sC' \cap C_X)_{\prec C'}$.
%%By the definition of $C'$, $q$ contains no non-collider in $\sC'$, 
%%and we have just proved that $p$ contains no non-collider $\sX'$.
%%So $q$ is active given $\lceil(\sX' \cup \sC')_{\prec C} \rceil$.
%%Hence $C' \prec Z$ from Lemma 1.
%%But this contradicts $Z \prec C'$.
%%So $p$ cannot contain any non-collider in $\sC'$.
%
%Proof of 4) %Now we prove that $p$ cannot contain a non-collider $Z \in \sZ$.
%Let $Z'$ be the non-collider in $\sZ$ nearest to $V$, and we will prove a contradiction.
%Let $q:V \overset{p}{\upathto} Z'$.
%For $p$ to be active, $Z'$ must be in $(\sV' \setminus \fix(C_X \setminus \sZ )_{\prec Z}$ or $\sV'_{\succ Z}$.
%The former is prohibited by $p$ being a shortest path, so $Z \prec Z'$.
%We know from activeness of $p$ that every collider in $q$ is in $\fix(C_X \setminus \sZ )_{\prec Z}$,
%and since $Z \prec Z'$, also in $\fix(C_X \setminus \sZ )_{\prec Z'}$.
%$q$ cannot contain any non-collider in $\sZ$ by the definition of $Z'$, 
%nor any non-collider in $\sX'$ or $\sC'$, as proved in (1,3).
%So $q$ is active given $\fix(C_X \setminus \sZ )_{\prec Z'}$.
%Moreover, $V \prec Z'$, since $V \prec Z$ and $Z \prec Z'$.
%Thus $p$ is not the shortest path 
%from $\sZ \ni Z' \upathto V \in (\sV' \setminus \fix(C_X \setminus \sZ ))_{\prec Z'}$
%active given $\fix(C_X \setminus \sZ )_{\prec Z'}$
%giving a contradiction.
%\Ryan{Actually, this just proves that $Z' \not \in \fix(C_X \setminus \sZ ))_{\succ Z'}$}
%
%We know that $p$ can only contain colliders in $\fix(C_X \setminus \sZ )$, and 
%these colliders cannot be in $\sX'$ or $\sZ$, by (1-2).
%Moreover, $\fix(C_X \setminus \sZ ) \cap \sC' = \sC' \cap C_X$, so 
%every collider in $p$ is in $\sC' \cap C_X$.
%From (1,3,4), we know that every collider is not in $\sV'$.
%\end{proof}
%
%\Ryan{Seems like this falls slightly short of saying that if $p$ is a Thm 1 violation, 
%then there must be a violation meeting these specific properties.
%Because the d-connecting path implies by the theorem does not necessarily have $Z \in C_X$.
%So the active path implied by the theorem may still be consistent with Thm 1.
%But I think this only applies to the proof of point (4), 
%so we do know that there is an active path of the sort described by (1-3) and also with $Z \in C_X \cap \sZ$
%(but that may contain a non-collider in $(\sZ \setminus C_X)_{\succ Z}$).
%}

\subsection{Analysing Thm 2}% [replaces ``simplifying thm 2'' and ``further thm 2'']}
%This raises some questions:
%    \begin{itemize}
%    \item Can I prove that decisions that are accumulated in some $n'>n$ cannot be used to observe variables in $p_n,q_n$? 
%    \item Is the activeness condition of $q_n$ strong enough to prevent there from being unintended ways to observe $Z$ and forks in $q$? 
%    \item Should I be concerned about chains of decisions from $Z$ to decisions in $p$? Will this mean that I need to reason about ``this $p,q$ cannot be solved without using decisions from outside''? Or could I modify $q$ to retrace those paths of decisions to somehow remove this issue?
%    \end{itemize}
\subsection{Introduction}

A natural next question is how this approach could be extended to Thm 2? Two ideas:
\begin{itemize}
        \item We could add an extra step to the construction of $\calH$. Then, the presence of a cycle would prove 
        some set of paths that we would parameterise to exhibit nonredundancy under optimality.
        \item Or, we could try to develop an algorithm that uses $\calH$ to select some $\prec$ to try to apply Thm 2.
        When the algorithm cannot find a suitable $\prec$, this must prove the presence of some paths, that we would parameterise.
\end{itemize}

Here is an example (\cref{fig:thm-2}) where we could try to deploy these approaches.
In this case, we can see that $Z$ is nonredundant under optimality because it provides information about $C$, which is not observed.
Thm 2 is unsatisfiable, because $C$ needs to be before $Z$ in order to satisfy Le 1.2, 
but it needs to be after $Z$ in order for $Z$ to be fixable.
Since $C$ and $Z$ are directly connected, we could describe this by simply adding another edge ($Z \to C$) to the ordering graph.
Or we can just prove that this problem will arise for any choice of ordering $\prec$ that is topological in the graph.
We could parameterise the graph using the edge $Z \to C$ as well as the paths $C \to Y$ and $X'' \to Y$ that are highlighted as usual.
But what if we try to extend this approach to the general case?
The problem arises that whether $Z$ is fixable is often not immediately apparent.
It depends on the ordering $\prec$ that is selected, of which the ordering graph often offers many choices.
What exactly a Thm 2 violation might look like is therefore quite variable.
So my next step was to analyse just how a Thm 2 violation can look.

\begin{figure} \label{fig:thm-2}
\centering
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv]  {$Z$};
%  \node (Xp) [rv,red,below = 16mm of Z]              {$X'$};
  \node (C) [rv, below right = 16mm and 16mm of Z,line width=0.6mm,dashed]  {$C$};
  \node (Xpp) [rv,red,below = 16mm of C,line width=0.6mm]              {$X''$};
  \node (X) [rv,red,left = 16mm of Xpp,line width=0.6mm]              {$X$};
  \node (Y) [rv, right = 16mm of Xpp]  {$Y$};

  
%\draw[->, very thick, color=black] (Z) -- (Xp);
  \draw[->, very thick, color=gray,dashed] (Z) to [bend right] (X);
  \draw[->, very thick, color=black] (Z) -- (Xpp);
%  \draw[->, very thick, color=black] (Xp) -- (C);
  \draw[->, very thick, color=black] (Z) -- (C);
%\draw[->, very thick, color=black,dashed] (C) -- (X);
  \draw[->, very thick, color=black] (C) -- (Xpp);
  \draw[->, very thick, color=black] (X) to [bend right] (Y);
  \draw[->, very thick, color=green] (Xpp) -- (Y);
  \draw[->, very thick, color=red] (C) -- (Y);
\end{tikzpicture}
\caption{A case where Le 1 is satisfiable (with $\sX'=\{X,X''\},\sC'=C,\sZ=Z$ and $\prec=\langle C,Z,X,X''\rangle$) but Thm 2 is not, because $\fix(\emptyset)=\emptyset \not \supseteq \{Z\}$.} \label{fig:thm-2-1}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (C) [rv]  {$C$};
  \node (Z) [rv, right=6mm of C]  {$Z$};
  \node (X) [rv,red,right = 6mm of Z]              {$X$};
  \node (Xpp) [rv,red,right = 6mm of X]              {$X''$};
  
  \draw[->, very thick] (C) -- (Z);
  \draw[->, very thick] (Z) -- (X);
  \draw[->, very thick] (X) -- (Xpp);
  \draw[->, very thick] (C) to [bend right] (Xpp);
\end{tikzpicture}
\caption{An ordering graph for $\sX'=\{X,X''\},\sC'=C,\sZ=Z$ and $\prec=\langle C,Z,X,X''\rangle$}
\end{subfigure}
\end{figure}



\subsection{Intermediate results}
In any case, to begin with, 
the conditionals of Thm 2, currently include a conditional independence statement.
This has two disadvantages: 1) usually, it is neater to use a criterion that is termed wholly in terms of the graphical structure
2) it's hard to know how exactly to prove completeness for a criterion that includes statements about non-graphical features.

So let's state a variation on Thm 2. that replaces the conditional independence statement with a d-separation statement.

\begin{theorem}
Let $\sU,\sZ,\prec$ satisfy Le 1.
Let $\hat{\sT}:= \lceil \sT\rceil \cup \{Z \in \sZ \mid \sV_Z \setminus \sU' \subseteq \lceil \sT \rceil \}$
where  $\sV_Z$ is a minimal subset of $\sV'_{\prec Z} \cup \sU'$ s.t. $\sZ \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sV_Z \mid \sV_Z$.
Let $\fix'(\sT)$ be the fixed point of $\hat{\sT}$.
Let $\calS':= (\calS \setminus \sX') \cup \{ \langle X,C_X \setminus \sZ \rangle \}_{X \in \sX'}$.
If $\fix'(C_X \setminus \sZ ) \supseteq C_X$ for all $X \in \sX$ then $\mu^*_{\calS'}=\mu^*_{\calS}$.
\end{theorem}

\begin{proof}
Whenever $\sZ \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sV_Z \mid \sV_Z$, then $Q(Z\mid \sV_Z)=Q(Z\mid \sV'_{\prec Z},\sU')$ (by soundness of d-sep)
so $\fix(\sW)\supseteq \fix'(\sW)$ for any variables $\sW$.
So $\fix'(C_X \setminus \sZ ) \supseteq C_X$ implies that $\fix(C_X \setminus \sZ ) \supseteq C_X$, 
which implies by Thm 2 that $\mu^*_{\calS'}=\mu^*_{\calS}$.
\end{proof}

This has just proved that Thm2b is immediate from Thm 2, as we intended it to be.

Now let us analyse Thm 2b. 
To begin with, we present a lemma that allows us to remove $\sV_Z$ from the conditional.

\begin{lemma} \label{le:no-need-minimal-subset}
Let $\sV_Z$ be a minimal subset of $\sV'_{\prec Z} \cup \sU'$ such that $Z \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sV_Z \mid \sV_Z$ and let $\sT \subseteq \sV'$.
Then $$\sV_Z \setminus \sU' \subseteq \lceil \sT \rceil \text{ iff }
Z \dsep (\sV'_{\prec Z} \setminus \lceil \sT \rceil) \mid (\sV'_{\prec Z} \cap \lceil \sT \rceil ) \cup \sU'.$$
\end{lemma}
\begin{proof}
\emph{Proof of $\Leftarrow$ direction.}
Let $\sW:=(\sV'_{\prec Z} \cap \lceil \sT\rceil)\cup\sU'$.
Then $\sW$ is a subset of $\sV'_{\prec Z} \cup \sU'$,
that has $Z \dsep (\sV'_{\prec Z} \cup \sU')\setminus \sW \mid \sW$,
and has $\sW \setminus \sU' \subseteq \lceil \sT \rceil$.
So the minimal subset $\sV_Z$ of $\sV'_Z \cup \sU'$ that has $Z \dsep (\sV'_{\prec Z} \cup \sU')\setminus \sV_Z \mid \sV_Z$
must be a subset of $\sW$, hence must also satisfy $\sV_Z \setminus \sU' \subseteq \lceil \sT \rceil$.

\emph{Proof of $\Rightarrow$ direction.}
If a minimal subset $\sV_Z$ of $\sV'_Z \cup \sU'$ that has $Z \dsep (\sV'_{\prec Z} \cup \sU')\setminus \sV_Z \mid \sV_Z$ 
also has $\sV_Z \setminus \sU' \subseteq \lceil \sT \rceil$, 
then the superset $\sW:=(\sV'_{\prec Z} \cap \lceil \sT\rceil)\cup\sU'$
will also have $Z \dsep (\sW \cup \sU')\setminus \sV_Z \mid \sW$ by \cref{le:move-endpoint-to-condset-preserves-sep}.
And clearly $\sW \setminus \sU' \subseteq \lceil \sT \rceil$, proving the result.
\end{proof}

This means that to see whether some $Z$ can be fixed (i.e.\ added to $\sT$), we do not need to check any minimal subset(s) of predecessor variables.
Instead, we can check whether the fixed predecessors $(\sV'_{\prec Z} \cap \lceil \sT \rceil )$ block all paths to unfixed predecessors.

The next step in our analysis is to specify the circumstances in which some $Z$ is not in $\fix'(C_X \setminus \sZ )$, 
i.e. is ``unfixable'').
In such cases, $Z$ must be connected to an unfixed predecessor.
Moreover, that unfixed predecessor must itself have a path to another unfixed predecessor, and so on.
The specifics of this chain of unfixed variables is as follows.

\begin{lemma} \label{le:z-to-unfixed-predecessor}
Assume that $\sZ,\sC',\sX',\sU',\prec$ satisfy Le 1.
For every $Z \in \sZ \setminus \fix'(C_X \setminus \sZ )$,
there exists a 
path $p:V \upathto Z$ that:
\begin{enumerate}
    \item is active given $\fix'(C_X \setminus \sZ )_{\prec Z} \cup \sU'$
    \item contains no $\sV' \setminus \fix'(C_X \setminus \sZ )_{\prec Z}$ except its endpoints
    \item contains no $\sU'$
    \item contains no $\sX'$ except possibly $V$
    \item contains no non-colliders in $\sC'$
    %\item contains no colliders in $\sZ$.
\end{enumerate}
\end{lemma}

\begin{proof}
(There is a path $p$ that satisfies 1-2)
Choose any $Z \in \sZ \setminus \fix'(C_X \setminus \sZ )$.
At the fixed point $\sT=\fix'(C_X \setminus \sZ)=\lceil \fix'(C_X \setminus \sZ) \rceil$, 
the minimal subset $\sV_Z$ of $\sV'_{\prec Z} \cup \sU'$ such that $\sZ \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sV_Z \mid \sV_Z$
has $\sV_Z \setminus \sU' \not \subseteq \fix'(C_X \setminus \sZ) $.
So, from \cref{le:no-need-minimal-subset}, 
$Z \not \dsep (\sV'_{\prec Z} \setminus \fix'(C_X \setminus \sZ) ) \mid (\sV'_{\prec Z} \cap \fix'(C_X \setminus \sZ) ) \cup \sU'$.
So there is a path from $Z$ to an unfixed predecessor $V \in (\sV'_{\prec Z} \setminus \fix'(C_X \setminus \sZ)$ 
that is active given $(\sV'_{\prec Z} \cap \fix'(C_X \setminus \sZ) ) \cup \sU'$.
Let $V'$ be the vertex nearest to $Z$ in $\sV' \setminus \fix'(C_X \setminus \sZ )_{\prec Z}$, 
and truncate the path at $V'$ to obtain $p$, which satisfies (1-2).

(Proof that $p$ satisfies 3)
The path $p:$ is active given a conditioning set that includes $\sU'$, so cannot contain any non-colliders in $\sU'$, 
and neither can there be colliders in $\sU'$ because the exogenous variables $\sU'$ contain no inbound edges.

(Proof that $p$ satisfies 4)
If $p:V\upathto Z \in \sZ$ contains a collider $X \in \sX'$, by (1),
$X \in \fix'(C_X \setminus \sZ )_{\prec Z}$.
Then, Le 1 implies that $\Pa^\calG_X \subseteq \sV'_{\prec Z}$.
Moreover, $\Pa^\calG_X \subseteq \fix'(C_X \setminus \sZ )_{\prec Z}$, since $X \in \fix'(C_X \setminus \sZ )_{\prec Z}$.
This would block $p$ and give a contradiction. So $p$ does not contain a collider $X \in \sX'$.
If instead $p$ contains a non-collider $X \in \sX' \setminus \{V\}$, then 
$X \not \in \sX' \cap \fix'(C_X \setminus \sZ )_{\prec Z}$ by (1), 
and $X \not \in \sX' \setminus \fix'(C_X \setminus \sZ )_{\prec Z}$, because $X$ is not an endpoint.
So $X \in \sX'_{\succ Z}$.
We also know that $V \prec Z$. If $\sW$ denotes the set of colliders in $p$, then we also know 
that $\sW \in \sV'_{\prec Z}$.
It follows from Le 1 that $X \not \in \Anc^\calG_{Z \cup V \cup \sW}$.
So $p$ cannot contain a non-collider $X \in \sX' \setminus \{V\}$.
Thus $p$ cannot contain any $X \in \sX' \setminus \{V\}$.

(Proof that $p$ satisfies 5)
Suppose for a contradiction that (5) is false, and then let $C'$ be the non-collider in $\sC'$ nearest to $Z$ on $p$.
Let $p':C' \overset{p}{\upathto} Z$.
Let $Z'$ be the collider in $\sZ$ nearest to $C'$ in $p'$ and let $q:C' \overset{p'}{\upathto} Z'$.
By (2), $p$
contains no $(\sV' \setminus \fix(C_X \setminus \sZ ))_{\prec Z}$.
And by (1), $C' \not \in \fix(C_X \setminus \sZ )_{\prec Z}$.
So $Z \prec C'$.
By (1), $Z' \prec Z$, so $Z' \prec C'$.
However, with Le 1, we will prove the opposite ordering for $Z'$ and $C'$.
By (1), every collider in $q$ is in $\fix'(C_X \setminus \sZ)_{\prec Z}$.
By (4), $q$ contains no collider in $\sX'$. %(except endpoints).
And, by the definition of $Z'$, $q$ contains no collider in $\sZ$.
So every collider in $q$ is in $\sC'$. 
By the definition of $\hat{\sT}$, $\sC' \cap \fix'(C_X \setminus \sZ)_{\prec Z}=(\sC' \cap C_X)_{\prec V_i}$.
So every collider in $q$ is in $(\sC' \cap C_X)_{\prec C'}$.
By the definition of $C'$, and (4), $q$ contains no non-collider in $\sC' \cup \sX'$,
so $q$ is active given $\lceil(\sX' \cup \sC')_{\prec C} \rceil$.
Hence $C' \prec Z'$ from Le 1.
This contradicts $Z' \prec C'$, so $p$ cannot contain a non-collider in $\sC'$.

%(Proof of 1f.)
%.....................................\ryan{proof of 1f still being transcribed}

\end{proof}

\begin{lemma} \label{le:x-to-unfixed-predecessor}
Assume that $\sZ,\sC',\sX',\sU',\prec$ satisfy Le 1.
For every $X \in \sX' \setminus \fix'(C_X \setminus \sZ )$,
there exists an edge
$p:V \to X$ 
such that $V \in \sV'_{\prec X} \setminus \fix'(C_X \setminus \sZ)$
\end{lemma}
\begin{proof}
Choose any $X \in \sX' \setminus \fix'(C_X \setminus \sZ)$.
$X \not \in \fix'(C_X \setminus \sZ)$ implies, by the definition of $\hat{\sT}$, that some parent of $X$ is not in $\fix'(C_X \setminus \sZ)$.
And Le 1 requires that the parents of $X$ that are not in $\sC' \cup \sX'$ are in $\sZ$, i.e.\ $\sV\ \supseteq C_X$.
So $X$ has a parent $V \in \sV' \setminus \fix'(C_X \setminus \sZ)$, which has $V \prec X$, by Le1.3.
\end{proof}

In \cref{le:z-to-unfixed-predecessor,le:x-to-unfixed-predecessor}, we
have proved that each node $V_n \in (\sZ \cup \sX') \setminus \fix'(C_X\setminus \sZ)$ 
has a path $p_n$ to a predecessor in $V_{n-1}\in (\sZ \cup \sX' \cup \sC')_{\prec V_n} \setminus \fix'(C_X\setminus \sZ)$.
If $V_{n-1} \not \in \sC'$, then we can also choose a path $p_{n-1}$ for $V_{n-1}$, iteratively, 
until we reach some vertex in $\sC' \setminus \fix'(C_X\setminus \sZ)$.
We can call that vertex $V_0$, and the set of paths $\{p_i\}_{1\leq n}$

\subsection{Current thoughts}
\begin{itemize}
    \item I have some tentative ideas about how to choose an ordering
    \item But I don't see an obvious way to choose the ordering between $Z$ nodes, especially when they are not all in $C_X$
\end{itemize}

==> sections/old/old-decision-on-control-path.tex <==
\begin{figure}[t]\centering
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0mm}, node distance=15mm, >=stealth]
  \node (Z) [rv, label=$Z_0 \sim U(\mathbb{B})$]  {$Z_0$};
  \node (X) [rv,red,below = 10mm of Z, label=below:{$=z_0$}] {$X_0$};
  \node (Zp) [rv,right = 10mm of X, label=below:{$=x_0$}] {$Z_1$};
  \node (Vp) [rv,below = 10mm of X] {$U_1$};
  \node (Xp) [rv,red,right = 6mm of Zp, label=below:{$=z_1$}] {$X_1$};
  \node (Y) [rv, right = 10mm of Xp,label={[xshift=-4mm,yshift=2mm]$y=\llbracket z_0=x_1 \rrbracket$}]  {$Y$};

  \draw[->, very thick] (Z) -- (X);
  \draw[->, very thick] (Z) -- (Xp);
  \draw[->, very thick] (X) -- (Zp);
  \draw[->, very thick] (Zp) -- (Xp);
  \draw[->, very thick] (Vp) -- (Zp);
  \draw[->, very thick, color=black] (Vp) to [bend right=15] (Y);
  \draw[->, very thick] (Xp) -- (Y);
  \draw[->, very thick,red] (Z) -- (Y);
\end{tikzpicture}
\caption{$Z_0$ is immaterial for $X_0$.}\label{fig:decision-on-control-path-no-voi}
\end{subfigure}
\begin{subfigure}[b]{0.55\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0mm}, node distance=15mm, >=stealth]
  \node (Z) [rv, label=$Z_0 \sim U(\mathbb{B})$]  {$Z_0$};
  \node (X) [rv,red,below = 10mm of Z, label={[xshift=5mm,yshift=-11mm]$=z_0$}] {$X_0$};
  \node (Zp) [rv,right = 10mm of X, label={[xshift=8.5mm,yshift=-11mm]$=\!\langle x_0, u_1[x_0] \rangle$}] {$Z_1$};
  \node (Vp) [rv,below = 10mm of X, xshift=5mm, label={[xshift=-3mm,yshift=-1mm]$u_1 \sim \mathbb{B}^2$}] {$U_1$};
  \node (Xp) [rv,red,right = 14mm of Zp, label={[xshift=6mm,yshift=-9mm]{$=z_1$}}] {$X_1$};
  \node (Y) [rv, right = 17mm of Xp,label={[xshift=-8mm,yshift=3.5mm,align=left]$y=\llbracket z_0=x_1[0] \rrbracket$ \\ $+ \llbracket u_1[x_1[0]]=x_1[1] \rrbracket$}] {$Y$};

  \draw[->, very thick] (Z) -- (X);
  \draw[->, very thick] (Z) -- (Xp);
  \draw[->, very thick] (X) -- (Zp);
  \draw[->, very thick] (Zp) -- (Xp);
  \draw[->, very thick,blue] (Vp) -- (Zp);
  \draw[->, very thick, color=black,blue] (Vp) to [bend right=10] (Y);
  \draw[->, very thick] (Xp) -- (Y);
  \draw[->, very thick,red] (Z) -- (Y);
\end{tikzpicture}
\caption{$Z_0$ is material for $X_0$.}\label{fig:decision-on-control-path-yes-voi}
\end{subfigure}
\caption[Materiality in simple one-two decision graphs]{Two models, constructed using a red info path, with and without the additional blue info path} \label{fig:decision-on-control-path}
\end{figure}

==> sections/old/old-if-child-is-decision-proofs.tex <==





\begin{lemma} \label{le:cannot-distinguish-n}
Let $\calM$ be a materiality SCM for $\calG_\calS$, 
where the child of $X_0$ along $d$, $\Ch^d(X_0)$ is a \emph{decision}.
Then, the truncated info path $m_1$ is not a directed path, and under any
deterministic policy $\spi$ in the scope $\langle X,C_X \rangle_{X \in \sX(\calS) \setminus X_0} \cup \langle X_0, C_{X_0} \setminus Z_0 \rangle$
that satisfies Conditions \cref{eq:2,eq:2b}, 
there must exist assignments 
%$A=a$,
$\Pa(Y^{\sp_1})=\pa(Y^{\sp_1})$, 
$C^{\neg m_1}_{X_0}=c^{\neg m_1}_{X_0}$
$X_0=x_0$, 
$\Pa(X_0^{m_1})=u$,
$\Pa(X_0^{m_1})=u'$
such that
\begin{itemize}
%\item $P^\spi(x_0 \mid \pa(Y^{\sp_1}),a)>0$
%\item $P^\spi(c^{\neg m_1}_{X_0},\pa(Y^{\sp_1}))>0$
\item $P^\spi(c^{\neg m_1}_{X_0},\pa(Y^{\sp_1}), x_0)>0$
\item $u[\pa(Y^{\sp_1})] \neq u'[\pa(Y^{\sp_1})]$
\item $x_0 = \pi_{X_0}(u,c^{\neg m_1}_{X_0})=\pi_{X_0}(u',c^{\neg m_1}_{X_0})$.
\end{itemize}
\end{lemma}
%\ryan{Does $A=a$ need to be in the support? If so, change it to $P(x_0,a \mid \pa(Y^{\sp_1})$?}
\ryan{Rename $N$ as $C^{m_1}_{X_0}$ in nro-paths?}
\ryan{Update $Pa_V$ to $Pa(V)$ throughout.}
\ryan{Bold $C_{X_0}$ throughout, as long as it is not referring only to one variable, like $C^{m_i}_{X_0}$}
\ryan{Check that what is proved corresponds to the itemize statements above, which match what is needed in the next lemma.}
\ryan{``Support'' -> 'has positive probability' where appropriate}
\ryan{$P^\spi(c^{\neg m_1}_{X_0},\pa(Y^{\sp_1}), x_0)$ -> $P^\spi(c^{\neg m_1}_{X_0},\pa(Y^{\sp_1}), x_0,u)$?}
\begin{proof}
By assumption, $X_1$ is the child of $X_0$ along $d$, so 
the info path $m_1$ must be of the form $Z_1 \gets C^{m_1}_{X_0} \upathto Y$ %where $C^{m_1}_{X_0} \in \sC_{Z_0} \setminus \condset{Z_1}$ 
(\cref{le:nro-paths}).
Let the parents of $X_0$ except $C^{m_1}_{X_0}$ be $\sC^{\neg m_1}_{X_0}:= \sC_{X_0} \setminus C^{m_1}_{X_0}$.


As $A^d$ assigns strictly positive probability to at least $2^k$ assignments, 
and $\Pa^d_Y \aseq A^d$ (by Condition \cref{eq:2b}), so does $\Pa(Y^d)$, 
and since $\sp_1\ni d$, so does $\Pa(Y^{\sp_1})$.
Meanwhile, $\sC^{\neg m_1}$ cannot intersect the control path, 
nor any portion of the info path except its colliders, by activeness.
This means $\sC^{\neg m_1}$ can only intersect portions of the materiality paths with domain $\bool$,
so the domain of $\sC^{\neg m_1}$ cannot be larger than $\lvert \dom{\sC^{\neg m_1}_{X_0} \setminus Z_0}\rvert \leq 2^{bc}$, 
where $b$ is the maximum number of variables belonging to any context $C_X$, and $c$ is the largest number of materiality paths passing through any vertex.
So, 
$\sfrac{\lvert \{\pa(Y^{\sp_1}):P^\spi(\Pa(Y^{\sp_1})=\pa(Y^{\sp_1})>0\})\rvert}{\lvert \dom{\sC^{\neg m_0}_{X_0} \setminus Z_0}\rvert} \geq 2^{k-bc}$. 

So, there exists
an assignment $\sC^{\neg m_1}_{X_0}=\sc^{\neg m_1}_{X_0}$
and a set of assignments $\dom{\Pa(Y^{\sp_1})}'$ of size at least $\lvert \dom{\Pa(Y^{\sp_1})}' \rvert \geq 2^{k-bc}$,
such that $\forall \pa(Y^{\sp_1} \in \dom{\Pa(Y^{\sp_1})}', P(\sC^{\neg m_1}_{X_0}=\sc^{\neg m_1}_{X_0}, \Pa(Y^{\sp_1})=\pa(Y^{\sp_1})>0$.

How large can the domain of $X_0$ be? 
$X_0$ intersects $d$, and the domain of $X_0^d$ is $k$ bits (\cref{def:nro-model}).
However, $X_0$ cannot intersect any of the truncated info paths, except the endpoint of $m_1$, and the colliders. 
So the info paths and collider paths can only contribute $c$ more bits to the domain of $X_0$, 
and hence $\dom{X_0} \rvert = k+c$.

............
By the definition of $k$, we have that $\lvert \dom{\Pa(Y^{\sp_1})}' \rvert \geq 2^{k-bc} > k+c \geq \dom{X_0}$.
So, given $\sC^{\neg m_1}_{X_0}=\sc^{\neg m_1}_{X_0}$, it is not possible for $\pi_{X_0}$ to map each $u \in \dom{\Pa(Y^{\sp_1})}'$ to a unique value.
So, there must exist $u,u' \in \dom{\Pa(Y^{\sp_1})}'$
such that:

\ryan{How do we prove the second bullet?}


$\pa(Y^{\sp_1}),c^{\neg m_1}_{X_0},x_0$
%$x_0 \in \supp (X_0 \mid \pa^{\sp_1}_Y,c^{\neg m_i}_{X_0})$
and $u,u' \in \dom{\Pa^{m_1}_{X_0}}$ 
such that
$P(c^{\neg m_1}_{X_0},\pa(Y^{\sp_1}), x_0)>0$, $u[\pa(Y^{\sp_1})] \neq u'[\pa(Y^{\sp_1})]$, and $x_0 = \pi_{X_0}(u,c^{\neg m_1}_{X_0})=\pi_{X_0}(u',c^{\neg m_1}_{X_0})$.
\end{proof}

%(i.e.\ sometimes the slices of $U_{i,0}$ at $\pa^{\sp_1}_Y$ must differ, if the function $f_{X_0}$ gives rise to the same assignment at $X_0$).
In other words, sometimes there will be an assignment $\pa^{\sp_1}_Y$ to the parent of $Y$ along $\sp_1$, 
and to $c^{\neg m_1}_{X_0}$, the parents of $X_0$ outside $m_1$, such that
$X_0$ fails to distinguish an important bit from $U_{1,1}$.
We can then prove that in this case, there exists an intervention to the fork variables $\sU_{1,1:\jmax^i}$
that does not affect $X_0$, but such that Condition \cref{eq:2} is no-longer satisfied.
%In this case, there must exist an assignment to colliders $\sW_{1,1:\jmax^i}$, 
%with $P(\pa^{\sp_1}_Y,a,x_0,\sw,\pa^{r_{1,1}}_Y)>0$.

\ryan{Move most of this (about the interventions on fork nodes) into the subsection above to match the theme there.}
\begin{lemma}[Required properties unachievable if child is a decision] \label{le:impossible-decision}
Let $\calM$ be the materiality SCM for some scoped graph $\calG_\calS$, 
where the child of $X_0$ along $d$, $V:=\Ch^d_{X_0}$ is a \emph{decision}.
Then, there exists no deterministic policy in the scope $\langle X,C_X \rangle_{X \in \sX(\calS) \setminus X_0} \cup \langle X_0, C_{X_0} \setminus Z_0 \rangle$
that satisfies Conditions \cref{eq:2,eq:4,eq:2b}.% for all $i$.
\end{lemma}


\begin{proof}
We will prove the result by contradiction, assuming that
a deterministic policy in the scope $\langle X,C_X \rangle_{X \in \sX(\calS) \setminus X_0} \cup \langle X_0, C_{X_0} \setminus Z_0 \rangle$ 
satisfies \cref{eq:2,eq:2b} and then showing that $\neg$\cref{eq:2}.
From \cref{le:cannot-distinguish-n}, $m_1$ is not a directed path, and, for any such deterministic policy,
there must exist assignments 
$\pa(Y^{\sp_1}),c^{\neg m_1}_{X_0},x_0$ and $u,u' \in \dom{\Pa^{m_1}_{X_0}}$ such that
$P(c^{\neg m_1}_{X_0},\pa^{\sp_1}_Y, x_0)>0$, $u[\pa^{\sp_1}_Y] \neq u'[\pa^{\sp_1}_Y]$, and $x_0 = f_{X_0}(u,c^{\neg m_1}_{X_0})=f_{X_0}(u',c^{\neg m_1}_{X_0}).$
Then, let $\sw$ be any assignment to the colliders $\sW_{1,1:\jmax^i}$ such that $P(\sw \mid c^{\neg m_1}_{X_0},\pa^{\sp_1}_Y, x_0)>0$.
Also, define an assignment to forks $\sU_{1,1:\jmax^i}$, $\su = \langle u,u_2,\ldots,u_\jmax^i \rangle$, where each $u_j$ consists of $w_j$ repeated 
$\lvert U_{i,j} \rvert$ times.
Define $\su'$ in the identical fashion, except with $u'$ replacing $u$.
Note that $u_2[u]=w_2=u_2[u']$ and for $j>2$, we have $u_j[u_{j-1}]=w_j$.
Then, we have:
\begin{align*}
0 &< P^\spi(\pa^{\sp_1}_Y,c^{\neg m_1}_{X_0},\sw,x_0) & (\text{From \cref{le:cannot-distinguish-n} and definition of $\sw$}) \\
\intertext{
Intervening $\doo(\su)$ can only have effects on $\Pa(Y^{\sp_1}),C^{\neg m_1}_{X_0},\sW_{1,1:\jmax^1},X_0$, 
1) through endpoints of $m_1$, 2) via contexts lying on $m_1$, or 3) if these variables lie on the path $m_1$.
We know that 1) is false, because $f_{X_0}(u,c^{\neg m_1}_{X_0})=x_0$, and the other endpoint $Y$ is a non-ancestor of these variables.
2) is false, because 
the colliders $W_{1,1:\jmax^1}$ have $u_2[u]=w_2$, and $u_j[u_{j-1}]=w_j$ for $j \geq 2$, and 
the context $C^{m_1}_{X_0}$ has $\sC_{X_0} \!\setminus\! \sC_{\sX(\calS)}$ by the the definition of the materiality paths (\cref{le:nro-paths}).
Finally, 3) is false, in that no variables other than $X_0$ and the colliders $W_{1,1:\jmax^1}$ can lie on $m_1$, because $m_1$ is active 
given $\condset{X_0}$ by the definition of the materiality paths.
So we have:
}
& = P^\spi(\pa^{\sp_1}_Y,c^{\neg m_1}_{X_0},\sw,x_0,\doo(\su),\pa^{r_{1,1}}_Y) & \\
& = P^\spi(\pa^{\sp_1}_Y,c^{\neg m_1}_{X_0},\sw,x_0,\su,\pa^{r_{1,1}}_Y) & (\text{Do calculus rule 2; $\sU_{i,1:\jmax^i}$ unconfounded}) \\
\intertext{Repeating these two steps with $\su'$ in place of $\su$, and using $f_{X_0}(u',c^{\neg m_1}_{X_0})=x_0$ and $u_2[u']=w_2$, we obtain:}
0 & < P^\spi(\pa^{\sp_1}_Y,c^{\neg m_1}_{X_0},\sw,x_0,\su',\pa^{r_{1,1}}_Y) & \\
\end{align*}
So we have an assignment 
$\pa(Y^{\sp_1}),u,\pa^{r_{1,1}}_Y$
in the support, which must have
$u[\pa(Y^{\sp_1})] = \pa(Y^{r_{1,1}})$ by \cref{eq:2}.
But then we also have the assignment 
$\pa(Y^{\sp_1}),u',\pa(Y^{r_{1,1}})$ in the support, 
which has $u'[\pa(Y^{\sp_1})] \neq u[\pa(Y^{\sp_1})]$ by assumption, 
and which then violates $\cref{eq:2}$.
So, condition \cref{eq:2} cannot be satisfied.





%\emph{Case 2: $\Ch^{d}_{X_0}$ is a decision.}
%The domain $\mathfrak{X}_{X_0}$ contains at most $k + c$ bits, where $c$ is the number of paths in the graph.
%So given an assignment $\pa^{\neg m_1}_{X_0}$ to parents of $X_0$ other than $\Pa^{m_1}_{X_0}$, there can only be $k+c$ different values $b$ 
%(where $b$ has the same size as the domain of paths incoming, $b \in \mathfrak{X}_{\sp_i}$) such that:
%\begin{equation} \label{eq:info-preserved}
%\text{ for every } \pa^{m_1},x_0 \text{ with } p(\pa^{m_1}[b], x_0)>0, \text{ we have } p(\Pa^{m_1}=1-\pa^{m_1}[b], x_0)=0.
%\end{equation}
%\ryan{this must be true, but not sure how best to prove it}
%Moreover, $\Pa^{\neg m_1}$ has a domain not larger than $\bool^c$.
%So there can be at most $(k+c)2^c$ different values such that \cref{eq:info-preserved} is true for any assignment to $\Pa^{\neg m_1}$.
%We know, however, that $\Pa(Y^{\sp_1})$ supports greater than $2^k$ different assignments \cref{le:full-support}.
%Moreover, $k$ was chosen to have $2^k > (k+c)2^c$.
%So there must exist some $\Pa(Y^{\sp_1})$ such that is false for every $\pa^{\neg m_1}_{X_0}$.
%Then, we can intervene the fork nodes $U_{1,j},j>1$ to prove that the policy performs suboptimally.
%Formally, let $w_{1,1},\ldots,w_{1,\jmax_1}$
%be an assignment such that 
%$P^\spi(\pa^{\neg m_i}(X_0))^{m_1}, \pa(Y^{\sp_1}), w_{1,1},\ldots,w_{1,\jmax_1})>0$.
%Then, there exists an assignment $v'_{1,1},\ldots,v'_{1,\jmax_1}$ 
%that leads to the same values for the $w_{1,j}$ variables, by \cref{le:encryption2}.
%So we intervene that assignment to obtain
%$P^\spi(\pa^{\neg m_i}(X_0))^{m_1}, \pa(Y^{\sp_1}),, w_{1,1},\ldots,w_{1,\jmax_1},\doo(v'_{1,1},\ldots,v'_{1,\jmax_1}))>0$.
%The fork variables lack any dependence on their parents, so we have \\
%{$P^\spi(\pa^{\neg m_i}(X_0))^{m_1}, \pa(Y^{\sp_1}),, w_{1,1},\ldots,w_{1,\jmax_1},v'_{1,2},\ldots,v'_{1,\jmax_1})>0$}, 
%and so task $1$ is not performed.


%Formally,
%$\mathfrak{X}_{X_0}$ has domain at most $\bool^{k+\text{num\_paths}}$ 
%(where $\text{num\_paths}$ is the maximum number of inbound paths in $\ss$ to any node)
%so
%given an assignment $\pa^{\neg m_i}(X_0)$ to parents of $X_0$ other than $\Pa(X_0^{m_1})$, 
%$f_{X_0}$ has
%for at most $k+\text{num\_paths}$ different values $m$ such that \ryan{define $\text{num\_paths}$ as the largest number of paths inboudn to any variable in the graph.}
%that
%for all $\pa(X_0^{m_1}) \in \mathfrak{X}_{\Pa(X_0^{m_1})}$
%$f_{X_0}(\pa(X_0^{m_1})[m], \pa^{\neg m_i}(X_0) \neq \pa'^{m_1}_{X_1}[m]$.
%Moreover, the support of $\Pa(Y^{\sb_1})$ is at least $\bool^k$, 
%and $2^k / 2^{\text{num\_paths}} > k + \text{num\_paths}$, 
%so there must be an assignment $\pa^{\neg m_i}(X_0)$ such that 
%more than k+\text{num\_paths} assignments to $\Pa(Y^{\sb_1})$
%have $P(\pa^{\neg m_i}(X_0), \Pa(Y^{\sb_1}))>0$.
%So there is at least one assignment with 
%$P(\pa^{\neg m_i}(X_0), \Pa(Y^{\sb_1}))>0$
%and 
%$f_{X_0}(\pa(X_0^{m_1})[m], \pa^{\neg m_i}(X_0) \neq \pa'^{m_1}_{X_1}[m]$
%for $m=\pa(Y^{\sb_1})$.
%That is to say that on occasion, $X_0$ does not distinguish the necessary bit from $U_{1,1}$.
\end{proof}

==> sections/old/old.tex <==
\begin{lemma}[Topological ordering implies d-separations 1]
Let $\calH'$ be the ordering graph for any $\calG,\sX',\sC',\sZ,Y$, and $\prec$ be any topological ordering over $\calH'$.
Then, $\sZ_{\prec C} \dsep_\calG C \mid \lceil (\sC' \cup \sX') \cap \text{Anc}^\calH_Z \rceil$ for all $C \in \sC' \cup \{Y\}$.
\end{lemma}
\begin{proof}

We will prove that d-connection cannot occur, because 
if there was any  walk $w$ from some $Z$ to some $C$ such that $Z \prec C$ that was active given $\lceil (\sC' \cup \sX') \cap \text{Anc}^\calH_Z  \rceil$, 
then it must also be active given $\lceil \sC' \cup \sX' \rceil$, so must already have been added to $\calH$.

Suppose there was a walk $w$ from some $Z$ to some $C$ that was active given $\lceil (\sC' \cup \sX') \cap \text{Anc}^\calH_Z  \rceil$, 
but that was not active given $\lceil \sC' \cup \sX' \rceil$.
Then, that must mean that a collider in $w$ is in $\lceil \sC' \cup \sX' \rceil$, but no non-colliders in $w$ are in $\lceil \sC' \cup \sX' \rceil$.
If all of these colliders are in $\sC$, then 
the for the $C' \in \sC$ nearest to $Z$, an edge $C' \to Z$ should be added to $\calH$, based on the definition of $h$.
This implies that $C'$ must be an element of $\Anc^\calH_Z$, and so it is in the conditioning set.
Then, the next collider $C''$ must have an edge $C'' \to Z$ in $\calH$, and so on.
By induction, there should be an edge $C \to Z$ in $\calH$.
Moreover, $\prec$ is topological in $\calH$ so 
this implies that there cannot be a walk $w$ from some $Z$ to a $C$ such that $Z \prec C$. \ryan{Break this inductive argument off into a Lemma.}

If, however, one or more of these colliders is in $\sX$, 
then consider the collider $X \in \sX$ nearest to $C$.
Then, based on the definition of $h$, there must be an edge $C' \to X$, and 
Then $X$ it should already have been added as a descendant of $C$ in $\calH$.

\ryan{I realise this bit is not solid yet}
So there cannot be any such collider, implying that there is a contradiction.
\end{proof}

==> sections/old/van-merwijk-scheme-dual.tex <==
\begin{figure}
\begin{subfigure}[t]{0.47\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
\node (Z0) [rv, label=0:{$\!\sim\! U(\bool)$}]  {$Z$};
\node (X0) [rv,red, below=9mm of Z0, label={[xshift=7.6mm,yshift=-4mm]$=z$}]              {$X$};
\node (Z1) [rv, right=12mm of X0, label={[xshift=11.6mm,yshift=-6mm]$=\langle z,x\rangle$}]              {$Z'$};
\node (X1) [rv,red, below=12mm of Z1, label={[xshift=12mm,yshift=-4mm]$=\langle z'$}]              {$X'$};
\node (W) [rv, below right=3mm and 8mm of Z1]              {$W$};
\node (V) [rv, right=22mm of Z1]              {$U$};
\node (Y) [rv, right=22mm of X1, label={[xshift=-13mm,yshift=-12.5mm,align=left]$y={\color{red}\llbracket x'[0]\!=\!x'[1]\rrbracket}$}]              {$Y$};
%\node (Y) [rv, right=16mm of X1, label={[xshift=21.1mm,yshift=-4mm,align=left]$=\delta (x^1=x^2)$ \\ + $\delta (w=v[x^1])$}] {$Y$};

  \draw[->, very thick] (Z0) -- (X0);
  \draw[->, very thick, red] (Z0) -- (Z1);
  \draw[->, very thick] (X0) -- (Z1);
  \draw[->, very thick] (Z1) -- (X1);
  \draw[->, very thick] (Z1) -- (W);
  \draw[->, very thick, red] (Z1) -- (X1);
  \draw[->, very thick] (V) -- (W);
  \draw[->, very thick] (V) -- (Y);
  \draw[->, very thick] (W) -- (X1);
  \draw[->, very thick, red] (X1) -- (Y);
\end{tikzpicture}
\caption{The \citet{everitt2021agent} scheme is applied using just the red info path; $Z$ is immaterial.} \label{fig:soluble-everitt}
\end{subfigure}\hspace{2mm}
\begin{subfigure}[t]{0.47\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
\node (Z0) [rv, label=0:{$\!\sim\! U(\bool)$}]  {$Z$};
\node (X0) [rv,red, below=9mm of Z0, label={[xshift=7.6mm,yshift=-4mm]$=z$}]              {$X$};
\node (Z1) [rv, right=12mm of X0, label={[xshift=11.6mm,yshift=-6mm]$=\langle z,x\rangle$}]              {$Z'$};
\node (X1) [rv,red, below=12mm of Z1, label={[xshift=12mm,yshift=-4mm]$=\langle z', w\rangle$}]              {$X'$};
\node (W) [rv, below right=3mm and 8mm of Z1, label={[xshift=9.6mm,yshift=-7mm]$=u[x']$}]              {$W$};
\node (V) [rv, right=22mm of Z1, label={[xshift=10mm,yshift=-4mm]$\sim U(\bool^4)$}]              {$U$};
\node (Y) [rv, right=22mm of X1, label={[xshift=-19mm,yshift=-12.5mm,align=left]$y={\color{blue}\llbracket x'[1] \!=\! u[x'[0]]\rrbracket} + {\color{red}\llbracket x'[0][0]\!=\!x'[0][1]\rrbracket}$}]              {$Y$};
%\node (Y) [rv, right=16mm of X1, label={[xshift=21.1mm,yshift=-4mm,align=left]$=\delta (x^1=x^2)$ \\ + $\delta (w=v[x^1])$}] {$Y$};

  \draw[->, very thick] (Z0) -- (X0);
  \draw[->, very thick, red] (Z0) -- (Z1);
  \draw[->, very thick] (X0) -- (Z1);
  \draw[->, very thick] (Z1) -- (X1);
  \draw[->, very thick, blue] (Z1) -- (W);
  \draw[->, very thick] (Z1) -- (X1);
  \draw[->, very thick, blue] (V) -- (W);
  \draw[->, very thick, blue] (V) -- (Y);
  \draw[->, very thick] (W) -- (X1);
  \draw[->, very thick] (X1) -- (Y);
\end{tikzpicture}
\caption{The \citet{van2022complete} scheme is applied, using the red and blue info paths; $Z$ is material.} \label{fig:van-merwijk-scheme}
\end{subfigure}
\caption{Two decision problems on a soluble graph.} \label{fig:soluble-past}
\end{figure}

==> sections/old/x-generalised-stepladder.tex <==
\section{More on the generalised stepladder (sequence of $p,q,\{r_i\}$ paths)}

\begin{lemma}
    $\calG^-$ is unique (i.e.\ if edges are added according to the procedure above, the resulting graph does not 
    depend on the order in which edges are added)
\end{lemma}
\begin{proof}
The key intermediate result is 
(1): if $A \to B$ may be added to $\calG$, a subgraph of $\calG'$, and $A \to B$ is not in $\calG'$, 
then $A \to B$ may also be added to $\calG'$.
\ryan{Actually, this is not quite correct. Seems like I should change the edge-addition condition so that the result is unique.}
%Proof of (1): if paths $p,q$ in $\calG$ allow $A \to B$ to be added, then 
%the same $p$ may be selected in a supergraph $\calG' \supseteq \calG$. 
%Then                                   $C_{\sXnew^{\cal{G}'}(p)} \setminus C \subseteq C_{\sXnew^{\cal{G}}(p)} \setminus C$.
%This means that $C \not \dsep_\calG Y \mid C_{\sXnew^{\cal{G}'}(p)} \setminus C$ (\autoref{le:active-to-ancestors-preserved-subset})
%Since $\calG \subseteq \calG'$, $C \not \dsep_{\calG'} Y \mid C_{\sXnew^{\cal{G}'}(p)} \setminus C$.
\end{proof}

Counterexample to the above lemma: ......


Now, I we prove that for any edge that is not in $\calG^-$, Le1 can be satisfied.
\begin{lemma}
Let $\calG^-$ be any fixed point from edge-addition as per the ``generalised stepladder'.
For any $Z \to X$ that is in $\calG \setminus \calG^-$,
there exists a $\sC'$, $\sX' \ni X$, $\sZ \ni Z$, $\sU, \prec$ that satisfies Lemma 1.
\end{lemma}

\begin{proof}
We will assume that Le 1 is unsatisfiable, and then prove the result by contradiction.

Choose
 \\
$\sC' = \{C':(C' \to X') \in \calG^-,X' \in \sX'\}$ \\
$\sX' = \{X':(C' \to X') \in \calG^-,X' \in \sX'\}$ \\
$\sZ = \{Z':(Z' \to X') \in \calG \setminus \calG^-, X' \in \sX'\}$.

If Le 1.1 is unsatisfiable given $\sC',\sX',\sZ$, t
hen there is a path $Z \upathto Y$ that is active given $\lceil \sX' \cup \sC' \rceil$.
This implies activeness given the subset $C_{\sXnew(p)} \setminus Z$, so that $Z \to X$ may be added to $\calG^-$, 
so $\calG^-$ is not a fixed point as assumed.

So assume instead that Le1.1 is satisfiable, but there exists no $\prec$ such that $\sC',\sX',\sZ,\prec$ satisfies Le1.2-1.3.
Then, there must be a cycle in the dependency graph $\calH$.
In the dependency graph, the only edges that are not of the form $V \to \Desc^\calG_V$ are those from some $C \in \sC'$
to some $Z \in \sZ$.............




\end{proof}



This means that for any edge that does not satisfy Le1, we have the following structure.

This seems tricky to parameterise because......

As side-points:
- There also exist some tricky cases:......
- One possible simplification would remove colliders.....

I wonder whether we could get a stronger condition, where at least part of $q$ is active given a larger set of variables.
This would help us to prove that variables cannot get information in unintended ways.


==> sections/old/y-beyond-stepladder.tex <==
\section{Beyond the stepladder}
Last meeting, I said that there seem to be problems with using a
``stepladder'' of directed \& M-paths for the case where Le1 is unsatisfiable.
I now have a more detailed picture of how this goes wrong, and 
present a more general approach.

\subsection{Stepladder unworkable for proving nonredundancy under optimality}
Per last meeting, I have a sketch that
if Lemma 1 cannot be satisfied with $\sZ \supseteq Z$ and $\sX \supseteq X$,
then $Z$ must lie at the top of a stepladder.
But this turns out not to be useful, if $X$ is not also in the stepladder.
In such scenarios:
\begin{enumerate}
\item $Z \to X$ is not assured to be NRO.
e.g.\ in \cref{fig:step-fail-1}, 
$Z$ is redundant under optimality for $X$ (not-NRO).
\item even when $Z \to X$ is NRO, the paths provided by the stepladder may be the wrong ones for proving NRO, e.g.\ in \cref{fig:step-fail-2}, 
the stepladder paths will not work for proving 
that $Z \to X$ is NRO because $C$ is observed by $X$.
Instead, a different suitable set of paths is illustrated.
A parameterisation scheme based on these paths is shown in
\cref{fig:step-fail-2-params}.
\end{enumerate}


\begin{figure} \centering
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv]              {$Z$};
  \node (Xpp) [rv,below=of Z,red]              {$X''$};
  \node (C) [rv,right=of Xpp]              {$C$};
  \node (Xp) [rv,below=of C,red]              {$X'$};
  \node (Y) [rv,right=of Xp]              {$Y$};
  \node (X) [rv,below=of Xpp,red]              {$X$};

  \draw[->, very thick, color=blue] (Z) -- (Xpp);
  \draw[->, very thick, color=yellow] (Z) -- (Xp);
  \draw[->, very thick, color=black] (Z) -- (C);
  \draw[->, very thick, color=yellow] (Z) to [bend right=35] (X);
  \draw[->, very thick, color=black] (Xpp) -- (C);
  \draw[->, very thick, color=blue] (C) -- (Xp);
  \draw[->, very thick, color=blue] (C) -- (X);
  \draw[->, very thick, color=black] (X) to [bend right=35] (Y);
  \draw[->, very thick, color=black] (Xp) -- (Y);
  \draw[->, very thick, color=black] (C) -- (Y);
\end{tikzpicture}
\caption{
There is a stepladder with diagonal $Z \to C \to Y$.
But this doesn't help us to exhibit NRO for $Z \to X$.
In fact, the yellow edges are both redundant under optimality (not-NRO).
Whereas the NRO edges are shown in blue.
}
\label{fig:step-fail-1}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv]              {$Z$};
  \node (Xpp) [rv,below=of Z,red]              {$X''$};
  \node (C) [rv,right=of Xpp]              {$C$};
  \node (Xp) [rv,below=of C,red]              {$X'$};
  \node (Y) [rv,right=of Xp]              {$Y$};
  \node (X) [rv,below=of Xpp,red]              {$X$};
  \node (W) [rv,right=5mm of X]              {$W$};
  \node (S) [rv,below left=7mm of W]              {$S$};

  \draw[->, very thick, color=blue] (Z) [bend left=3] to (Xpp);
  \draw[->, very thick, color=red] (Z) [bend right=3] to (Xpp);
  \draw[->, very thick, color=red] (Z) -- (C);
  \draw[->, very thick, color=blue] (Z) to [bend right=35] (X);
  \draw[->, very thick, color=black] (Xpp) -- (C);
  \draw[->, very thick, color=blue] (Xpp) [bend left=3] to (Y);
  \draw[->, very thick, color=red] (Xpp) [bend right=3] to (Y);
  \draw[->, very thick, color=black] (C) -- (Xp);
  \draw[->, very thick, color=black] (C) -- (X);
  \draw[->, very thick, color=black] (Xp) -- (Y);
  \draw[->, very thick, color=blue] (X) -- (W);
  \draw[->, very thick, color=blue] (W) [bend left=1] to (Xp);
  \draw[->, very thick, color=green] (W) [bend right=1] to (Xp);
  \draw[->, very thick, color=green] (S) -- (W);
  \draw[->, very thick, color=green] (S) -- (Y);
  \draw[->, very thick, color=blue] (Xp) [bend left=3] to (Y);
  \draw[->, very thick, color=green] (Xp) [bend right=3] to (Y);
  \draw[->, very thick, color=red] (C) -- (Y);
\end{tikzpicture}
\caption{
To exhibit NRO for $Z \to X$, the stepladder with diagonal $Z \to C \to Y$ is of little use, because $C \in \Pa_X$.
Instead, we need the blue step, with two different ``sub-steps'' in red and green.
}
\label{fig:step-fail-2}
\end{subfigure}
\caption{Another tricky-to-parameterise graph (left) and a sample from the parameterisation (right)}
\end{figure}

\begin{figure} 
\includegraphics[width=15cm]{step-fail-2-params.jpg}
\caption{.}\label{fig:step-fail-2-params}
\end{figure}

In particular, I note three things about the paths in \cref{fig:step-fail-2}:
a) The ``base'' of the blue step, $Y$, is not the ``top'' of any other step,
b) The path for each $C \to X$ is chosen not to traverse any $C '\in C_X \setminus Z$, 
e.g.\ blue path (chosen for $Z \to X$) avoids $C$,
green path (chosen for $W \to X'$ avoids $C$),
but each path is allowed to traverse parents of other decisions, e.g.\ 
the red path can traverse $C$.
c) the paths still have acyclic dependencies, in the sense that 
the blue path passes through $Z \to X''$ (which is the ``root'' of the red path)
and through $W \to X'$, which is the root of the green path, but otherwise, 
the paths never pass through the root of any other step.

\subsection{A revised approach}
With these observations in mind, we can generalise the stepladder approach.
We still use the logic that an edge $C \to X$ is ``useful'' to observe because of a certain directed path $X \pathto Y$ and an M-path $C \upathto Y$, forming a ``step''.
And we still incrementally ``include'' more edges into the set of ``useful'' edges by adding additional steps.
But we change the activeness condition that is required for each of the M-paths.

Formally, suppose we're identifying which edges are nonredundant under optimality (NRO) in a graph $\calG$ induced by a scope $\calS = \langle X,C_X \rangle_{X \in \sX}$.
Let $\calG^-_0$ be $\calG$ but without every edge $C \to X$ that is incoming to a decision $X \in \sX$.
Then, obtain $\calG^-_i$ from $\calG^-_{i-1}$ by adding any edge $C \to X$
such that there exist paths 
$p:X \pathto Y$ in $\calG$
and $q:C \upathto Y$ in $\calG^-_{i-1}$
where $q$ is active in $\calG^-_{i-1}$ given $C_{\sXnew} \setminus \{C\}$, 
where $\sXnew = X \cup \{X' \in \sX \mid V \to X' \in p \text{ and } V \to X' \not \in \calG^-_{i-1}\}$.
When no more edges may be added, call resulting graph is $\calG^-$.

\Ryan{How do I prove that $\calG^-$ is unique?}

The intuition is that each time we choose a ``step'' that includes some $C \to X$, we can use it to ensure that information is passed along $C \to X$, 
in this respect, we are ``opening up'' that edge.
Then, whenever we obtain a new step at $C' \to X'$, the directed and $M$ paths can only include edges that have already been ``opened up''.
On the other hand, an edge $C \to X$ cannot be opened up if it has a step in $\calG$, but not in $\calG^-$.
%This means that $C \to X$ can only be ``opened up'' if another edge $C' \to X'$ is opened up, 
%which itself is not in $\calG^-$.
This means that $X$ only needs to use $C$ if $X'$ uses $C'$ and vice versa.
In these cases, Thm 2 should be able to prove that the edges $C \to X$ and $C' \to X'$ are redundant under optimality.b

That is, the hope is that this algorithm can find paths for all of the edges that are NRO, and those edges that are left are redundant under optimality.

If this works out, it would fix both problems identified with the stepladder approach:
(1): it works for some edges that do not lie in a regular stepladder, and
(2): it will select the right paths for us to exhibit NRO.

Of course, the precise formulation given may be incorrect.
But this process does at least seem to identify good paths for many NRO edges (and does not choose paths for non-NRO edges).
We can consider \cref{fig:step-fail-1,fig:step-fail-2}.

\begin{figure} \centering
\begin{subfigure}[b]{0.42\textwidth}\centering
\includegraphics[width=6cm]{algo-1.jpg}
\caption{
$C \to X'$ may be added to $\calG^-$, using the M-path $C \to Y$.
}
\label{fig:algo-1}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}\centering
\includegraphics[width=6cm]{algo-2.jpg}
\caption{
No edges may be added to $\calG^-$.
}
\label{fig:algo-2}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}\centering
\includegraphics[width=6cm]{algo-3.jpg}
\caption{
Edges may be added to $\calG^-$ in the sequence:
$C' \to X'$, $X' \to X''$, $C'' \to X''$, $Z \to X$.
}
\label{fig:algo-3}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}\centering
\includegraphics[width=25mm]{algo-4.jpg}
\caption{
Edges may be added to $\calG^-$ in the sequence:
$Z \to X'$, $X' \to X$.
}
\label{fig:algo-4}
\end{subfigure}
\caption{In each case, NRO edges are purple. 
In each case, they can be sequentially added to $\calG^-$.
Edges that are redundant under optimality are yellow, and can be made to satisfy Lemma 1.
}
\end{figure}

The next two steps are:
\begin{enumerate}
    \item Can we prove that this process adds all NRO edges (i.e.\ that all edges not in $\calG^-$ can be removed by satisfying Le 1?
    \item Can we prove from the existence of these types of paths, that the edges are NRO?
\end{enumerate}

Presently, I'm focusing on (1). I have a proof sketch that all edges not in $\calG^-$ satisfy Le1.1. 
Roughly, $\sC'$ and $\sX$ correspond to the contexts and decisions that are in $\calG^-$ but not $\calG^-_0$, i.e.\ those that are in the generalised step-ladder,
while $\sZ$ corresponds to the contexts that are in $\calG$ but not $\calG^-$, i.e.\ those that are not in the generalised step-ladder.

\newpage

==> sections/old/y-le1-old.tex <==
\clearpage\newpage
\section{Case where Le1 is unsatisfiable (Ordering graph)}
Now, let us proceed to the more general case where
% where Cond1 may or may not be satisfiable, 
% and 
Le1 is unsatisfiable.

First, we prove a simplified statement of Lemma 1:
\begin{lemma} \label{le:simplified-le1}
Given an MPS $\calS$, which satisfies non-redundancy (Thm. 1), let $\sX' \subseteq \sX(\calS)$, actions of 
interest, $\sC' \subset \sC_{\sX'} \setminus \sX$, non-action context of interest. If there exists a subset of exogenous variables
$\sU'$ in $\calG_\calS$, a subset of endogenous variables $\sZ$ in $\calG_\calS$, disjoint with $\sC\cup \sX'$, and subsumes
$\sC_{\sX'}\setminus (\sC'\cup \sX')$, and an order $\prec$ over $\sV'=\sC'\cup\sX'\cup\sZ$ such that:
\begin{enumerate}
\item $(Y \dsep \spi_{\sX'} \mid \lceil \sX' \cup \sC'\rceil)_{\calG_\calS}$
\item $(C \dsep Z_{\prec C},\sU' \mid \lceil (\sX' \cup \sC')_{\prec C} \rceil)_{\calG_\calS}$ for every $C \in \sC'$, and
\item $\sV'_{\prec X}$ is disjoint with $\Desc(X)_{\calG_\calS}$ and subsumes $\Pa(X)_{\calG_\calS}$ for every $X \in \sX'$,
\end{enumerate}
then, the expected reward for $\spi$, a deterministic policy optimal with respect to $\calS$, can be writen as:
$\mu_\spi=\sum_{y,\sc',\sx'}yQ'_{\sx'}(y,\sc')\sum_{\su',\sz}Q(\su')\prod_{Z\in\sZ}Q(z\mid\sv'_{\prec Z,\su'}\prod_{X\in\sX'}\pi(X\mid\sc_x)$.
\end{lemma}
\begin{proof}
This result differs from Le 1 in the COMP paper only in that it does not require that 
$C \dsep \spi_{\sX'_{\prec C}} \mid \lceil (\sX' \cup \sC')_{\prec C}\rceil)_{\calG_\calS}$ (*).
So it will suffice to prove that points 2-3 of this lemma imply (*).
Our approach is to prove that point 3 and $\neg$(*) implies $\neg$(2).
If $\neg$(*), then 
there is a path $p$ from
$C$ to $\pi_X \in \spi_{\sX'_{\prec C}}$, active given $\lceil (\sX' \cup \sC')_{\prec C}\rceil)_{\calG_\calS}$.
Since $X\in \sX'_{\prec C}$, $X$ is in the conditioning set, so $p$ must end with $V \to X \gets \pi_X$.
Moreover, $X \prec C$, and point 3 implies that $V\prec X$, so $V \prec C$.
So $V$ cannot be in $\sX' \cup \sC$, otherwise it would be in the conditioning set, blocking $p$.
So $V\in\sZ$. 
So by truncating $p$ at $V$, we have $C \not \dsep Z_{\prec C} \mid \lceil (\sX' \cup \sC')_{\prec C} \rceil)_{\calG_\calS}$, 
proving the result.
\end{proof}


Our approach will be to encode the requirements that Lemma 1 places on $\prec$ (and hopefully also that Thm 2 places) in a graph, 
where any topological ordering satisfies their conditions.
Then, we will be able to deduce that if the graph contains a cycle, the cycle in this ordering graph will imply the presence of 
some set of paths in the original graph $\calG_\calS$.


%\begin{figure}
%    \centering
%    \begin{subfigure}{.4\textwidth}\centering
%    \begin{tikzpicture}
%    
%    \end{tikzpicture}
%    \caption{$\calG$}
%    \end{subfigure}\hfill
%    \begin{subfigure}{.4\textwidth}\centering
%    \begin{tikzpicture}
%    
%    \end{tikzpicture}
%    \caption{$\calH$}
%    \end{subfigure}\hfill
%    \caption{Ordering graph example}
%\end{figure}


\begin{definition}[Ordering graph ($\calH$)]
Let $\bar{\calH}$ be the graph with vertices
$\sC',\sX',\sZ,\sU',\{Y\}$
with an edge $A \to B$ if 
\begin{itemize}
    \item[i)] (contexts to decision) $A \in$ $\Pa^\calG_B$ and $B\in \sX'$,
    \item[ii)] (decision to descendants) $A\in \sX'$ and $B \in$ $\Desc^\calG_A \setminus \{A\}$, or
    \item[iii)] (exo to endo) $A \in \sU'$ and $B \not \in \sU'$.\slee{To be precise, we would not have explicit nodes for exogenous variables. Further, there would be no constraint created by iii) U to V since the lemma focuses on $\prec$ over $\mathbf{V}'$...} %ryan: U' mentioned here
\end{itemize}
\slee{We didn't define $\bar{\calH}$ yet.Further, the reason why we define $h(\bar{\calH})$ is not given. I am replacing $h()$ to $\calH$}\ryan{The idea was that the argument of $h$ starts as $\bar{\calH}$, and then changes at each step until we reach the fixed point $\calH$. I've tried writing it again, but feel free to improve it.}

Then, define an operation $h(\calH')$ as follows.
If $\calG$ contains a path $p:Z\upathto C$, 
from any $C \in \sC', Z \in \sZ \cup \sU' \setminus \Pa^{\bar{\calH}}_C$,
that is active given 
$\lceil (\sC' \cup \sX') \cap \Anc^{\bar{\calH}}_{Z \cup C} \rceil$ and active given $\lceil \sC' \cup \sX' \rceil$, 
then $h$ chooses arbitrarily such a path $p:Z \upathto C$, and adds the edge $C \to Z$ to $\calH'$.
Otherwise, $h$ returns $\calH'$.
Let $\calH$ be the fixed point of $h(\bar{\calH})$.

%Then, we define $\calH$ as follows:
%\[
%\calH = 
%\begin{cases}
%(\sV_{\bar\calH},\sE_{\bar\calH} \cup (C \to Z)) & \text{if $\calG$ contains a path $p:Z\upathto C, C \in \sC', Z \in \sZ \cup \sU' \setminus \Pa^{\bar{\calH}}_C$, active } \\  %ryan: U' mentioned here
% &\qquad\text{given } \\
%\bar{\calH}& \text{otherwise}.
%\end{cases}
%\]
% \slee{For just some pair $C$ and $Z$?}\ryan{fixed.} \slee{Check also $\Anc^\calH$. is it $\Anc^{\bar{\calH}}$?}\ryan{yes, fixed}
%(When multiple $C \in \sC, Z\in\sZ \cup \sU'$ satisfy the condition, we choose $C,Z$ arbitrarily.)\slee{Would be nice to be incorporated in $h(\cdot)$ clearly.}

%Then let $\calH'' = h(\calH')$.

\ryan{Maybe we could add more edges to the ordering graph to address Thm 2?}
%Define
%$$h'(\bar{\calH}) = 
%\begin{cases}
%(\sV_{\bar\calH},\sE_{\bar\calH} \cup (Z \to C)) & \text{if $\calG$ contains a path $p:C\upathto Z, C \in \sC', Z \in \sZ \setminus \Ch^{\bar{\calH}}_C$, active } \\ 
% &\qquad\text{.............} \\
%\bar{\calH}& \text{otherwise}
%\end{cases}
%$$
%again, breaking ties arbitrarily.
%
%Then, the \emph{full ordering graph} is defined as $\calH=h'(\calH'')$.
\end{definition}


\slee{Shouldn't we start by assuming that $\calH$ does not contain a cycle to define a topological ordering?}\ryan{I added ``there exists''. Better?}
\begin{lemma}
If $\sX',\sC',\sZ$ satisfy Cond1.1
and there exists a topological ordering $\prec$ over $\calH$, restricted to $\sX',\sC',\sZ$, 
then Cond 1 is satisfied by $\sX',\sC',\sZ,\sU',\prec$ (i.e.\ Cond1.2 and Cond1.3 are also satisfied) %ryan: \sU' mentioned here
\end{lemma}

\begin{proof}
It is immediate that any topological ordering over $\calH$, restricted to $\sX',\sC',\sZ$
satisfies Cond1.3, 
because
$\calH$ is defined to contain an edge
$C \to X$ for each parent
$C \in \Pa^\calG_X$ of every decision $X \in \sX'$ 
and an edge 
$X \to V$
for each descendant
$V \in \Pa^\calG_X$, of every decision $X \in \sX'$.

Now we prove that any topological ordering over $\calH$, restricted to $\sX',\sC',\sZ$
satisfies Cond1.2.
First, let us derive a more convenient formulation of Cond1.2. We derive from a version of the d-separations that does not contain $\spi$, as per \cref{le:simplified-le1}.
\begin{align*}
& \forall C \in \sC' : \sZ_{\prec C},\sU' \dsep^\calG C \mid \lceil(\sX' \cup \sC')_{\prec C} \rceil \\
\Longleftrightarrow & \forall C \in \sC' \forall Z \in (\sU' \cup \sZ)_{\prec C} : Z \dsep^\calG C \mid \lceil(\sX' \cup \sC')_{\prec C} \rceil && [\sU'_{\prec C} = \sU' \text{ by def.\ of } \calH] \\
%\Longleftrightarrow & \forall C \in \sC' \forall Z \in (\sU' \cup \sZ)_{\prec C} : Z \dsep^\calG C \mid \lceil(\sX' \cup \sC')_{\prec C} \cup (\sX' \cup \sC')_{\prec Z} \rceil && [\text{quantifying over } Z \prec C]\\
\Longleftrightarrow & \forall C \in \sC' \forall Z \in \{Z' \in \sU' \cup \sZ \mid Z' \not \dsep^\calG C \mid \lceil(\sX' \cup \sC')_{\prec C}\rceil\} : C \prec Z.&& [\text{contrapositive}]
%\Longleftrightarrow & \forall C \in \sC' \forall Z \in \{Z' \in \sU' \cup \sZ \mid Z' \not \dsep^\calG C \mid \lceil(\sX' \cup \sC')_{\prec C} \cup (\sX' \cup \sC')_{\prec Z'}\rceil\} : C \prec Z.&& [\text{contrapositive}]
\end{align*}
%\ryan{Maybe makes more sense to move the bit about quantifying over $Z \prec C$ into the proof section below}
\footnote{slee: Given that $Z\prec C$, $(\sX' \cup \sC')_{\prec Z} \subsetneq  (\sX' \cup \sC')_{\prec C}$. Hence, the derivation seems a bit redundant to include $(\sX' \cup \sC')_{\prec Z}$... This is regardless of whether the order is from $\calH$ or not. 
\ryan{I've tentatively removed it! I \emph{think} everything is still valid.}
}
So it will suffice to prove that 
whenever there is a path $p$ from
$C \in \sC'$ to $Z \in \sZ$ that is d-connected given
$\lceil (\sX' \cup \sC')_{\prec C} \rceil$,
we have $C \prec Z$.

The proof requires some definitions. 
Let $\sW := (\sX' \cup \sC')_{\prec C}$.
%We know that there is a path $p$  from $Z$ to $C$, active given $\lceil \sW \rceil$.
For each collider $V$ in $p$, let $q_V$ be a shortest path (which can be empty) from $V$ to $\lceil \sW \rceil$,\footnote{slee: note that $\lceil \sW \rceil\setminus \sW$ will not be in the shortest path BTW. It seems that you already have a lemma ancestors-of-closure.}
and let $w$ be the walk obtained by inserting segments $q_V$ into $p$.%
%as (i.e., explicitly visiting the given variable responsible for activating each collider in $p$)
\footnote{BTW, I once used collider-minimal shortest path \ryan{Is this online?} which might be useful (or not) here... Changed second $W$ to be $W'$ \ryan{Cool}}\[w:Z\overset{p}{\upathto} V_1 \overset{q_{V_1}}{\pathto} W \overset{q_{V_1}}{\pathfrom} V_1 \overset{p}{\upathto} V_2 \cdots V_n \overset{q_{V_n}}{\pathto} W' \overset{q_{V_n}}{\pathfrom} V_n \overset{p}{\upathto} C.\]

If $w$ does not contain any element of $\sX'$, we let $Z'=Z$.
If, $w$ contains one or more elements of $\sX'$, then let 
$X'$ be the element of $\sX'$
% \footnote{slee: specified $\in \sX'$. Based on Proof of (2), should it be $X'$?\ryan{Thanks, changing to $\sX'$ is correct}}
closest in $w$ to $C$, and let $Z'$ be parent of $X'$ that is closest to $C$.

We can now prove $C \prec Z$ by proving two subclaims:
\begin{itemize}
    \item[(1)] $Z'$ always exists\ryan{Added this, to make the proof more correct.}, and has $Z' \preceq Z$ 
    or $Z' \prec C$
    , and
    \item[(2)] $C \prec Z'$ \ryan{Updated this to be clearer.}
%is in $\Anc^\calH_{\{Z',C\}}$. 
\end{itemize}

\paragraph{Proof of (1)}\textbf{(Case: $w$ contains no element of $\sX'$)} In this case, $Z'=Z$ so $Z$ exists and has $Z'\preceq Z$.

\textbf{(Case: $w$ contains some $X \in \sX'$)}
$X'$ must be either an ancestor in $\calG$ of either an endpoint, or of a collider. 
By the definition of $w$ and $q_V$, every collider in $w$\footnote{slee: $w'$??? \ryan{I'm referring to $w$ here}} is in the conditioning set,
so $X' \in \Anc^\calG_{C \cup Z \cup \lceil \sW \rceil}$, 
So, by \cref{le:ancestors-of-closure}, $X \in \Anc^\calG_{\{C, Z\} \cup \sW}$, 
i.e.\ $X \in \Anc^\calG_{C \cup Z \cup (\sX' \cup \sC')_{\prec C}}$.
Hence $X' \in \Anc^\calH_{C \cup Z}$ by the definition of $\calH$. 
Since $X' \in \sX'$, this means that $X' \in \sW$.
Since $w$ is made of active paths given $\sW$ and shortest-paths to $\sW$, it follows that $X'$ can only be a collider in $w$.
Thus $X'$ has parents in $w$, so $Z'$ exists.
That $X' \in \Anc^\calH_{C \cup Z}$ also implies that $X \prec C$ or $X \prec Z$.
From $Z' \in \Pa^\calG_X$ we also have $Z' \in \Anc^\calH_X$, so $Z' \prec C$ or $Z' \prec Z$, proving (1).

\paragraph{Proof of (2)}
We know that $\prec$ is topological on $\calH$, so to prove that $C \prec Z'$, it will suffice to prove that $\calH$ contains $C \to Z'$.
We do this by induction. 
Denote as $C_1,...,C_n=C$ the variables in $\sC'$ in the the walk segment $w': Z' \overset{w}{\upathto}C$.%
\footnote{slee: overset $w'$? \ryan{I am using this notation to mean ``let $w'$ be the segment of $w$ from $Z'$ to $C$'', so I mean overset $w$ here}}%
\footnote{excluding $C$ itself? \ryan{Clarified: possibly equal} or `first` based on $Z'$ \ryan{Clarified: the one nearest to $Z'$}}
% \footnote{If prove by contradiction, should we say that it does \textbf{not} in the ancestors? \ryan{Yes, fixed.}}
We will prove that if  $C_i \in \Pa^\calH_{Z'}$ for every $i<n$, then $C_n \in \Pa^\calH_{Z'}$.
To see this, note that the segment $Z'\overset{w'}{\upathto}C_n$ does not contain:
\begin{itemize}
    \item any $X \in \sX' \setminus X'$ (because $X'$ was assumed to be the nearest node to $C$ in $\sX'$), nor
    \item any non-collider $C_i \in \sC'$ (because for $i<n$, we have $C_i \in \Pa^\calH_{Z'}\cap \sC' \subseteq \sW$, 
%so have $C'' \prec C'$ or $C'' \prec Z$ 
%and hence $C_i \in \sW$, 
which 
cannot occur at a non-collider, since $p$ is active given $\sW$ and each $q_V$ is a shortest path to $\sW$).
\end{itemize}
This means that every non-collider in $w'$ does not contain $\lceil \sW \rceil$.
Since any collider in $Z' \overset{w'}{\upathto}C_n$ is not in $\sX'$, it must be in $\sC'$.
So by assumption, it is in $\Pa^\calH_{Z'}$, and therefore in $\sW$.
So if we remove the directed portions $\{q_V\}_V$ from $Z' \overset{w'}{\upathto}C_n$, 
we have a path that is active given both $\lceil (\sX' \cup \sC') \cap \Anc^\calH_{\{C, Z\}} \rceil$ and $\lceil \sW \rceil$.
By the definition of $\calH$, this implies that $\calH$ contains $C_n \to Z'$.%
%This contradicts the assumption that $C'' \not \in \Anc^\calH_{\{C,Z\}}$,
\footnote{$Z$ or $Z'$? \ryan{$Z'$, which proves (2), and then (1-2) imply that $C \prec Z$ also. This should be clearer now.}}
By induction on $i=0,...,i=n$, we have that $\calH$ contains $C \to Z'$.

Then, using (1) and (2), we know that we cannot have $C \prec Z' \prec C$, so we must have $C \prec Z' \preceq Z$, proving the result.\ryan{Added this to explain how (1-2) are combined}
\end{proof}
\ryan{Need to account for $\sU'$ as analogous to $\sZ$.}



But what exactly does the presence of a cycle in $\calH'_i$ imply?
First we characterise the $Z \to C$ edges.
\begin{lemma}
If $w:V^1\upathto V^2$ is active given $\sA$ and active given $\sB$
then it is active given every subset 
$\sA \subseteq \sV \subseteq \sB$.
\end{lemma}
\begin{proof}
Every collider is in $\sA$, so is active given any $\sV \supseteq \sA$.
Every noncollider does not contain $\sB \supseteq \sV$ 
so is active given any $\sV$.
\end{proof}



==> sections/old/y-le1.1-unsatisfiable-no-decision.tex <==
%\section{Updated (rough) sketch of proof elements and uncertainties}
%\subsection{Why certain paths exist when Le 1 is unsatisfiable}
%If Le1 is unsatisfiable, then:
%For every $Z$, $\calG$ contains paths:
%\begin{enumerate}[label=(\alph*)]
%\item $Z \upathto Y$, active given $\lceil C_X \cup X \setminus Z \rceil$ and $X \pathto Y$ (b/c of nonredundancy).
%\item For some $C \in (C_X \cup Y)\setminus \sX$, paths $Z \upathto C$, active given $\lceil C_\sX \cup \sX \setminus Z \rceil$ and $X \pathto C$ 
%for some $X \in \sX$.
%(b/c otherwise $\calH$ acyclic given $\sZ=Z, \sX'=\sX$ and Le1 satisfied).
%\end{enumerate}
%
%Note that for (b), we do not get to choose the $X$. \ryan{I noticed this subtlety in the last few days.}
%
%If we assume that for every $Z$, Le1.1 is unsatisfiable, then we can say more:
%\begin{enumerate}[label=(c)]
%\item there is a $\Pi_X \to X \gets Z \upathto Y$, 
%active given $\lceil \sX \cup (C_\sX \setminus Z) \rceil$
%for \emph{every} $X \in \sX \cap \Ch_Z$. (b/c of the d-connectivity property of Le1.1, plus \cref{le:max-cond-satisfies-1.1})
%For this path to be active, $Z \not \in \sX$.
%\end{enumerate}

\section{The case where Le1.1 is unsatisfiable}
We consider the case where a node is non-redundant (Thm 1) and does not satisfy the first condition of Lemma 1 (henceforth `Le 1.1'). 
Precisely speaking, given $\calS$, for every $\sX'\subseteq \sX(\calS)$ and every $\sC' \subsetneq \sC_{\sX'}\setminus \sX'$, $\parens{Y \not\perp \spi_{\sX'}} \mid \lceil{\sX'\dotcup\sC'}\rceil_{\calG_\calS}$.
It will be helpful for us to assume that for \emph{every} $X$ and \emph{every} $Z \in C_X$, $Z$ does not satisfy Le1.1.

\slee{Can we prove whether the reduction is reasonable,}
\[
\forall_{X\in \sX(\calS)}\forall_{Z\in \sC_X}(Y \not\perp \spi_{X} \mid \lceil{\set{X}\dotcup \sC_X \setminus \set{Z}\rceil})_{\calG_{\calS}} \Longleftrightarrow 
\forall_{\sX'\subseteq \sX(\calS)}\forall_{\sC' \subsetneq \sC_{\sX'}\setminus \sX'} \parens{Y \not\perp \spi_{\sX'} \mid \lceil{\sX'\dotcup\sC'}\rceil}_{\calG_\calS}.
\]



\paragraph{A Simple Example}
One such graph can be seen in \cref{fig:causal-graph-3}.
% Can we again find an active path and a directed path to exhibit that $Z$ is nonredundant?
% Well, we can choose an M path from $Z$ to $W$ to $V$ to $Y$.
Consider an active path $Z\to W \gets V \to Y$.
% But 
% There are ways that $X_1$ can obtain information about $Z$ astep from that M-path.
% In particular, we will find it necessary to restrict the dimensionality of some of the decision variables.
% If we do not restrict the dimensionality of $X^2$, then $X^2$ will reconstruct $V$ as much as possible and pass the information to $X^1$. 
% If, however,
Let $X^2$ be binary and $Z$ be high-dimensional. Then, $X^1$ may use some information from $Z$.
Using this idea, it is possible to parameterise the graph so that $Z$ is nonredundant under optimality. 
% \slee{But in the example, $Z$ and $X^2$ are both binary.}

\begin{figure} \centering
\begin{subfigure}[b]{0.5\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (1) [rv,red,label=below:$\in \mathbb{B}^2$]              {$X^1$};
  \node (Z) [rv, above = 2.8cm of 1,label=$z \sim \mathbb{B}$]  {$Z$};
  \node (Y) [rv, right=2.2cm of 1,label=below:{$y=\llbracket v[x^1[0]]=x^1[1]\rrbracket$}] {$Y$};
  \node (V) [rv, above = 2.8cm of Y,label=above:$v \sim \mathbb{B}^2$]  {$V$};
  \node (3) [rv,red, above right= 0.6cm and 0.8cm of 1,label=right:$\in \mathbb{B}$] {$X^2$};
  \node (W) [rv, above = 0.6cm of 3,label={$w=v[z]$}]  {$W$}; %

  \draw[->, very thick, color=gray] (Z) -- (1);
  \draw[->, very thick, color=red] (Z) -- (W);
  \draw[->, very thick, color=red] (V) -- (W);
  \draw[->, very thick, color=red] (V) -- (Y);
  \draw[->, very thick, color=black] (W) -- (3);
  \draw[->, very thick, color=black] (Z) -- (3);
  \draw[->, very thick, color=green] (1) -- (Y);
  \draw[->, very thick, color=black] (3) -- (1);
\end{tikzpicture}
\caption{
The given parameterisation shows that $Z$ is nonredundant.
} 
\label{fig:causal-graph-3}
\end{subfigure}%
\begin{subfigure}[b]{0.5\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (1) [rv,red,label=below:{$=01$}]              {$X^1$};
  \node (Z) [rv, above = 2.8cm of 1,label={$z =0$}]  {$Z$};
  \node (Y) [rv, right=2.2cm of 1,label=below:{$y=\llbracket 1=1 \rrbracket=1$}] {$Y$};
  \node (V) [rv, above = 2.8cm of Y,label=above:{$v=10$}]  {$V$};
  \node (3) [rv,red, above right= 0.6cm and 0.8cm of 1,label=right:{$=1$}] {$X^2$};
  \node (W) [rv, above = 0.6cm of 3,label={$w=1$}]  {$W$}; %

  \draw[->, very thick, color=gray] (Z) -- (1);
  \draw[->, very thick, color=red] (Z) -- (W);
  \draw[->, very thick, color=red] (V) -- (W);
  \draw[->, very thick, color=red] (V) -- (Y);
  \draw[->, very thick, color=black] (W) -- (3);
  \draw[->, very thick, color=black] (Z) -- (3);
  \draw[->, very thick, color=green] (1) -- (Y);
  \draw[->, very thick, color=black] (3) -- (1);
\end{tikzpicture}
\caption{
A sample from the graph to the left\\ \null
} 
\label{fig:causal-graph-4}
\end{subfigure}
\caption{Another tricky-to-parameterise graph (left) and a sample from the parameterisation (right)}
\end{figure}

% \subsection{Choosing functions for some important paths}
\subsection{Parametrisation with No Decision as Context}\label{sec:para-no-dec-con}
% 

% What about a more general case?
To begin with, let us assume that Le1.1 is unsatisfiable for every $Z\in C_X$ for every $X\in\sX'$, and that every $Z \in C_X$ is a non-decision. %\slee{rewrote}
% \footnote{slee: It seems that Le 1.1 is only about $\sX'$ and $\sC'$. Le 1.1 starts with $\sX'$ and $\sC'$, given by a user. Thus, when we say, `Le1.1 is unsatisfiable', we are focusing on some $\sX'$ and $\sC'=\sC_{\sX'}$ w/ every context non-decision.}
\[
(Y \not\dsep \spi_{X}) \mid \lceil \set{X} \cup \sC_X\setminus \set{Z}\rceil)_{\calG_\calS}.
\]
% From \cref{le:max-cond-separates}, 
There is an active path from every $Z \in C_X$ to $Y$ given $\lceil \sX' \cup \sC' \setminus \{Z\} \rceil$ through $\pi_X \to X \gets Z \dotsc Y$ since otherwise it is contradictory as other paths $\pi_X\to X \gets C$ for $C\in \sC_X\setminus\set{Z}$ are blocked.
% \slee{can be understood roughly as applying (ii) in Thm 1 repeatedly}
% There also exists a path $X \pathto Y$ by the assumption of nonredundancy.

Let $Z_0, X_0$ be $Z,X$.
There exist paths $p_0:X_0 \pathto Y$ and $q_0:Z_0 \upathto Y$. 
By assumption that no decision as context, every decision $X_i \in \sX$ other than $X_0$ in $p$ is preceded by some $Z_i \not \in \sX$ without passing $X_0$\footnote{\slee{``without passing $X_0$'' This step needs a proof (seems easy).}}. 
%\slee{unless $X_i\to Y$. Also do you ignore variables other than $\sX$, $Y$, and contexts?} \ryan{I don't understand what you mean about $X_i \to Y$. I am just talking about the parent of $X_i$ in $p$, not talking about $\prec$.}\slee{got it, not every decision, but those in $p$}
Then we have a path $q_i:Z_i \upathto Y$ without passing $X_i$.
%
This is illustrated as in \cref{fig:le1.1-generalisation}.

%\begin{figure}
%\includegraphics[width=8cm]{1.1-unsatisfiable.jpg}
%\caption{.}
%\end{figure}
%\ryan{TODO: change to tikz}



\begin{figure} 
\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (X0) [rv,red]              {$X_0$};
  \node (Z0) [rv, above = 8mm of X0]  {$Z_0$};
  \node (N0) [rv, above = 28mm of X0]  {$V_{0,0}$};
  \node (Y) [rv, right=100mm of X0] {$Y$};
  \node (NJ) [rv, above = 28mm of Y]  {$V_{0,N_0}$};
  \node (W1) [rv, below right = 3mm and 20mm of N0]  {$W_{0,1}$}; %
  \node (Ndots) [rv, right = 44mm of N0,draw=none]  {\ldots};
  \node (WJ) [rv, right = 44mm of W1]  {$W_{0,N_0}$};
  
  \node (Z1) [rv, right=12mm of X0] {$Z_1$};
  \node (X1) [rv, red, right=8mm of Z1] {$X_1$};
  \node (Xdots) [rv, right=12mm of X1,draw=none] {\ldots};
  \node (ZI) [rv, right=12mm of Xdots] {$Z_I$};
  \node (XI) [rv, red, right=8mm of ZI] {$X_I$};
  
  \node (N10) [rv, below left = 12mm and 0mm of Z1] {$V_{1,0}$};
  \node (W1dots) [rv, above right = 2mm and 8mm of N10,draw=none] {\ldots};
  \node (N1J) [rv, below right = 2mm and 8mm of W1dots] {$V_{1,N_1}$};

  \node (NI0) [rv, below right = 12mm and 0mm of ZI] {$V_{I,0}$};
  \node (WIdots) [rv, above right = 2mm and 8mm of NI0,draw=none] {\ldots};
  \node (NIJ) [rv, below right = 2mm and 8mm of WIdots] {$V_{I,N_I}$};

  \draw[->, very thick, color=red,dashed] (N0) -- (Z0);
  \draw[->, very thick, color=gray] (Z0) -- (X0);
  \draw[->, very thick, color=red,dashed] (N0) -- (W1);
  \draw[->, very thick, color=red,dashed] (Ndots) -- (W1);
  \draw[->, very thick, color=red,dashed] (Ndots) -- (WJ);
  \draw[->, very thick, color=red,dashed] (NJ) -- (WJ);
  \draw[->, very thick, color=red,dashed] (NJ) -- (Y);
  \draw[->, very thick, color=black,dashed] (W1) -- (X0);
  \draw[->, very thick, color=black,dashed] (WJ) -- (Y);
  \draw[->, very thick, color=green,dashed] (X0) -- (Z1);
  \draw[->, very thick, color=green,dashed] (Z1) -- (X1);
  \draw[->, very thick, color=green,dashed] (X1) -- (Xdots);
  \draw[->, very thick, color=green,dashed] (Xdots) -- (ZI);
  \draw[->, very thick, color=green,dashed] (ZI) -- (XI);
  \draw[->, very thick, color=green,dashed] (XI) -- (Y);
  
  \draw[->, very thick, color=black,dashed] (N10) -- (Z1);
  \draw[->, very thick, color=black,dashed] (N10) -- (W1dots);
  \draw[->, very thick, color=black,dashed] (N1J) -- (W1dots);  
  \draw[->, very thick, color=black,dashed] (N1J) -- (Y);  

  \draw[->, very thick, color=black,dashed] (NI0) -- (ZI);
  \draw[->, very thick, color=black,dashed] (NI0) -- (WIdots);
  \draw[->, very thick, color=black,dashed] (NIJ) -- (WIdots);  
  \draw[->, very thick, color=black,dashed] (NIJ) -- (Y);  
  
\end{tikzpicture}
\caption{Note that each path from $W_i$ can intersect with $X_0 \pathto Y$ at any step of it, whereas we have shown the paths intersecting at arbitrary locations.} \label{fig:le1.1-generalisation}
\end{figure}



In addition to paths $p_0$ and $\{q_i\}_i$,  % just as in the previous approach.
% We specify $\{r_{j,i}\}$, the paths for each collider $W_{j,i}$ in $q_i$, in a new fashion: 
% \[r_{j,i} = 
% \begin{cases}
% W_{j,i}\overset{SP(W_{j.i},X_i)}{\pathto} X_i \overset{p_0}{\pathto} Y & \text{ if } W_{j,i} \in \Anc_{X_i} \\
% W_{j,i}\overset{SP(W_{j.i},Y)}{\pathto} Y & \text{ otherwise}
% \end{cases}\]
we specify paths for each collider $W_{i,j}$ in $q_i$, denoted by $\{r_{i,j}\}$: 
\[r_{i,j} = 
\begin{cases}
W_{i,j}\overset{SP(W_{i,j},X_i)}{\pathto} X_i \overset{p_0}{\pathto} Y & \text{ if } W_{i,j} \in \Anc_{X_i} \\
W_{i,j}\overset{SP(W_{i,j},Y)}{\pathto} Y & \text{ otherwise}
\end{cases}\]
\slee{Since $\set{X}\cup \sC_{X}\setminus\set{Z}=\set{X_0}\cup \sC_{X_0}\setminus\set{Z_0}$ are the only given and they are the ancestors of $X_0$ (parents and itself), any collider is ancestors of $X_0$. Further, $X_i$ are those in the directed path from $X_0$ to $Y$ in $p_0$. Hence, $W_{i,j}\in \Anc_{X_i}$ holds true for every $i$ and $j$. Am I correct?}


% \paragraph{Parametrization}
Let $N_i$ be the number of colliders in $q_i$.
If $q_i$ contains $N_i+1$ fork nodes, then designate them, beginning from the $Z_0$ end, as $V_{i,0}, V_{i,1}, \ldots V_{i,N_i}$.
If instead, $q_i$ has $N_i$ forks, then let $V_{i,0}=Z_0$ and let the forks be $V_{i,1}, \ldots V_{i,N_i}$.
\slee{There is an actual number of forks in $q_i$. You cannot say ` $N_i+1$ fork nodes in $q_i$' or `$N_i$ fork nodes in $q_i$'. there must be a condition. Does it depend on $Z_i \gets $ or $Z_i\to $?}
\ryan{fixed}
% \slee{Do you also consider bidirected edges?} \ryan{Good point, I haven't talked about that, but here is an argument why extending to that case might be easy: bidirected edges into a decision can't happen, because we're looking at the graph after we apply an MPS. If we have a bidirected edge to a non-decision, we can obtain a hidden variable DAG by replacing every A<--->B with A<---N--->B, and choose CPDs in the hidden variable DAG. Then we do the latent projection operation to obtain probability distributions on the original ADMG.} \slee{Does $j$ start from 0 or 1? How do you assign index $j$ on $q_i$ precisely?} \ryan{Clarified.}
Let  $V_{0,j}$ %\ryan{I've changed $F$ to $V$ to clarify that it is a fork node.}
sample ${2^{j}}$ random bits, %\slee{Do you mean $2^{j}$ bits?} \ryan{yes, clarified}
and $W_{i,j}=V_{i,j}[V_{i,j-1}]$, 
where $a[b]$ denotes the $b\textsuperscript{th}$ bit of $a$, where the index $b$ is in binary
(e.g.\ $1234[10]=3$).\footnote{\slee{Thanks for the clarification. I prefer the right-most bit being called the 0th bit. But it's okay.}}
Moreover, we write $Y=\sum_{i=0}^{I} Y_i$, where each $Y_i$ is equal to $1$ if $V_{i,N_i}$ does not contradict by the bits passed along (from $X_i$), and $0$ otherwise. \slee{what is the max $Y$ value? $I$ or $I+1$?}



%\begin{figure} 
%\includegraphics[width=8cm]{ladder-1.jpg}
%\caption{We're trying to prove that $Z \to X$ is nonredundant under optimality, 
%but the unsatisfiability of Le 1 still allows for the possibility that the only ``stepladder'' comes from a different decision $X' \neq X$.}\label{ladder-1}
%\end{figure}
%\begin{figure} 
%\includegraphics[width=6cm]{ladder-2.jpg}
%\caption{.}\label{ladder-2}
%\end{figure}
%\begin{figure} 
%\includegraphics[width=6cm]{ladder-3.jpg}
%\caption{.}\label{ladder-3}
%\end{figure}
%\ryan{TODO: change to tikz}

Moreover, each $r_{i,j}$ is a directed path that copies one bit. Specifically, every node that is not a decision $\sX(\calS )$ or $Y$ is equal to its parent in $r_{i,j}$, 
and each decision node has one bit in its domain \slee{The domain of $X\in\sX(\calS )$ is all one bit?}.
%In a slight variation from previously, we say that 
Let $k$ be the number of paths $r_{i,j}$ that contain $Z_i$.
Then each $V_{i,j}$ randomly samples $2^{i+k+j+1}$ bits. \slee{$V_{0,j}$ sample $2^j$ bits. It does not match $2^{i+k+j+1}$ even with $i=k=0$. }
The bits $i+1$ are accumulated from each $q_i$ path, and the bits $k$ are accumulated from the $r_{i,j}$ paths.
The bits $j$ are because each subsequent $V_{i,j}$ node is indexed by $V_{i,j-1}$.
%and some number of additional bits for any$q_i$
%i.e.\ decisions on $p$ are incentivised to pass along all the information they receive.
% \slee{Sanghack: It would be helpful to have a small but concrete example which clearly states $W$ and $V$ variables together with the number of bits associated with each variable.}\ryan{I've formalised this and added a couple of examples below.}

\slee{It would be clearer to write as a function, how many bits, or what is copied, etc.}
\begin{align*}
    V_{i,j} &=  \ldots \\  
    Z_i &=  \ldots   \\
    X_i &=  \ldots   \\
    Y_i &= \ldots 
\end{align*}


\begin{figure}[H]
\centering
\begin{subfigure}[b]{0.45\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (X0) [rv,red, label={[xshift=7.1mm,yshift=-4.5mm]$\in \bool^2$}]              {$X_0$};
  \node (Z0) [rv, above = 8mm of X0, label=0:{$=\!v_{0,0}$}]  {$Z_0$};
  \node (V0) [rv, above = 28mm of X0, label=0:{$\sim \bool$}]  {$V_{0,0}$};
  \node (Y) [rv, right=37mm of X0, label={[xshift=3mm,yshift=-17mm,align=left]$=\delta(v_{0,1}[x_1[1]]=x_1[2])$\\$+\delta(v_{1,0}[x_1[1,2]]=x_1[3])$}] {$Y$};
  \node (V1) [rv, above = 28mm of Y, label=0:{$\sim \bool^2$}]  {$V_{0,1}$};
  \node (W1) [rv, below right = 8mm and 14mm of V0, label=0:{$=\!v_{0,1}[v_{0,0}]$}]  {$W_{0,1}$};
  \node (Z1) [rv, right=8mm of X0, label={[xshift=6mm]$=x_0,v_{1,0}[x_0]$}] {$Z_1$};
  \node (X1) [rv, red, right=6mm of Z1, label={[xshift=7.1mm,yshift=-4.5mm]$\in \!\bool^3$}] {$X_1$};
  
  \node (V10) [rv, below left = 8mm and 4mm of Z1, label=0:{$\sim \bool^4$}] {$V_{1,0}$};

  \draw[->, very thick] (V0) -- (Z0);
  \draw[->, very thick] (Z0) -- (X0);
  \draw[->, very thick] (V0) -- (W1);
  \draw[->, very thick] (W1) -- (X0);
  \draw[->, very thick] (V1) -- (W1);
  \draw[->, very thick] (V1) -- (Y);
  \draw[->, very thick] (X0) -- (Z1);
  \draw[->, very thick] (Z1) -- (X1);
  \draw[->, very thick] (X1) -- (Y);
  
  \draw[->, very thick] (V10) -- (Z1);
  \draw[->, very thick] (V10) -- (Y);  
\end{tikzpicture}
\caption{An example of the parameterisation where an $r$ path passes through $X_0$}
\end{subfigure}\hspace{7mm}
\begin{subfigure}[b]{0.45\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (X0) [rv,red, label={[xshift=7.1mm,yshift=-4.5mm]$\in \bool$}]              {$X_0$};
  \node (Z0) [rv, above = 8mm of X0, label=0:{$=\!v_{0,0}$}]  {$Z_0$};
  \node (V0) [rv, above = 28mm of X0, label=0:{$\sim \bool$}]  {$V_{0,0}$};
  \node (Y) [rv, right=37mm of X0, label={[xshift=3mm,yshift=-17mm,align=left]$=\delta(v_{0,1}[x_1[1]]=w_{0,1})$\\$+\delta(v_{1,0}[x_1[1]]=x_1[2])$}] {$Y$};
  \node (V1) [rv, above = 28mm of Y, label=0:{$\sim \bool^2$}]  {$V_{0,1}$};
  \node (W1) [rv, below right = 8mm and 14mm of V0, label=0:{$=\!v_{0,1}[v_{0,0}]$}]  {$W_{0,1}$};
  \node (Z1) [rv, right=8mm of X0, label={[xshift=6mm]$=x_0,v_{1,0}[x_0]$}] {$Z_1$};
  \node (X1) [rv, red, right=6mm of Z1, label={[xshift=7.1mm,yshift=-4.5mm]$\in \!\bool^2$}] {$X_1$};
  
  \node (V10) [rv, below left = 8mm and 4mm of Z1, label=0:{$\sim \bool^2$}] {$V_{1,0}$};

  \draw[->, very thick] (V0) -- (Z0);
  \draw[->, very thick] (Z0) -- (X0);
  \draw[->, very thick] (V0) -- (W1);
  \draw[->, very thick] (W1) -- (Y);
  \draw[->, very thick] (V1) -- (W1);
  \draw[->, very thick] (V1) -- (Y);
  \draw[->, very thick] (X0) -- (Z1);
  \draw[->, very thick] (Z1) -- (X1);
  \draw[->, very thick] (X1) -- (Y);
  
  \draw[->, very thick] (V10) -- (Z1);
  \draw[->, very thick] (V10) -- (Y);  
\end{tikzpicture}
\caption{An example of the parameterisation where an $r$ path passes through $X_0$}
\end{subfigure}
\caption{We illustrate how the dimensionality of $V_{1,0}$ is greater in (a) where the $r$ path passes through $Z_1$.} \label{fig:le1.1-two-decisions}
\end{figure}

==> sections/old/y-stepladder.tex <==
\subsection{A stepladder of paths}
We want to prove that for edges that do not satisfy Le 1, 
they have certain properties.
Specifically, that there exists a set of paths that 
describe why that edge is nonredundant, given that 
some other edges are already known to be nonredundant.

To do this, we begin with a graph $\calG^-_0$ that is 
equal to $\calG$, except that it lacks all 
inbound links to decisions.
For each $\calG^-_i$, we will add back (``accumulate'') some of these missing 
edges.

Given each step, $\calG^-_i$, we must check whether we need to accumulate more 
edges.
To do this, we compute $\sZ,\sC',\sX'$,
such that every non-accumulated edge is in $\sZ \ni Z \to X \in \sX'$,
and use the ordering graph $\calH_{\sZ,\sC',\sX'}$
to check whether Le 1 is satisfied.
If Le 1 is satisfied, then we end the procedure, 
knowing that every non-accumulated edge is a candidate for removal.
Otherwise, we know there is a cycle in $\calH_{\sZ,\sC',\sX'}$, 
and use this fact to accumulate more edges.

We want the procedure for adding an edge to tell us as much as 
possible about that edge, based on the cyclicity of $\calH_{\sZ,\sC',\sX'}$.

First, we prove a few general consequences of such a cycle.

\begin{lemma}[Consequences of $\calH$-cycle] \label{le:consequences-of-h-cycle}
If some $\sZ,\sC',\sX'$ cannot satisfy Le 1 (with any $\prec$), then either:
\begin{enumerate}
\item $\sZ \not \dsep Y \mid \lceil \sC' \cup \sX' \rceil$; or
\item $\exists Z \in \sZ, C_j \in \sC' \cap \Desc^\calG_Z, C_i \in \sC' \setminus (\Anc^\calG_{C_j} \setminus C_j)$ s.t.
$Z \not \dsep C_i \mid \lceil \sC' \cup \sX' \rceil \setminus \{C_i\}$, %ryan: need to make sure the setminus C_i is in the H definition.
%ryan: reverse the ordering of C_i and C_j.
\end{enumerate}
\end{lemma}

\begin{proof}
If Le1.1 is violated, then (1) follows, proving the result.
If Le1.1 is satisfied, but Le 1 is unsatisfiable (with any $\prec$), 
then Le 1.2-1.3 is unsatisfiable, meaning $\calH_{\sZ,\sC',\sX'}$ contains a cycle.
Every edge $A \to B$ in $\calH$ where $A \not \in \sC',B \not \in \sZ$
has $B \in \Desc^\calG_A$, and $\calG$ is acyclic, so 
any cycle in $\calH$
must contain one or more edges $\{C_i \to Z_i\}_{i<K}$ 
where $C_i \in \sC'$ and $Z_i \in \sZ$.
From the acyclicity of $\calG$, one of these source variables $C_i$ 
must not be a $\calG$-ancestor of any others, $\forall i \neq j, C_i \not \in \Anc^\calG_{C_j}$.
The $\calH$-edge $C_i \to Z_i$ implies, from the definition of $\calH$ that 
$Z \not \dsep C_i \mid \lceil \sC' \cup \sX' \rceil \setminus \{C_i\}$.

Since $C_i \to Z_i$ is in a cycle in $\calG$, we have $Z_i \in \Anc^\calH_{C_i}$, 
so we may let $C_j$ be the first element of $\sC'$ in the $\calH$-path
$p:Z_i \pathto C_i$.
For every edge $V_i \to V_{i+1}$ in this initial segment of p, 
$V_{i+1} \in \Desc^{\calG}_{V_i}$, so $C_i \in \Desc^{\calG_{V_i}}$.
As we have proved, if $j \neq i$, then $C_j \not \in \Anc^\calG_{C_j}$, 
proving the result.
\end{proof}

%ryan: {Add picture?

If we have a procedure for choosing $\sZ,\sX',\sC$ from 
an accumulated graph $\calG^-_n$ then this will yield
an inductive procedure for accumulating more edges.
Specifically, suppose we can let $\sZ$ and $\sX'$ be the sources and destinations of any non-accumulated edge (i.e.\ any candidate for removal), and let $\sC$ be the other contexts.
\begin{definition}
\begin{align*}
\bar{\sZ}=\{Z: Z \to X \in \calG \setminus \calG^-_n\}\\
\bar{\sX}'=\{X: Z \to X \in \calG \setminus \calG^-_n\}\\
\bar{\sC}'=\Pa^\calG_{\sX'} \setminus \bar{\sZ}
\end{align*}
\end{definition}

\begin{lemma} \label{le:stepladder}
Let $\calG^-_0$ be the result of removing from $\calG$, 
the inbound edges to every decision $X \in \sX$.
Then, there is a sequence of graphs 
$\calG^-_0,...,\calG^-_n,...\calG^-_N$ such that
\begin{enumerate}
\item There exists some $\sZ,\sX',\sC'$ 
such that every edge $Z \to X$ in $\calG \setminus \calG^-_N$ has $Z \in \sZ,X\in\sX'$
and $\sZ,\sX',\sC'$ satisfies Lemma 1; and
\item for $n>1$, every $\calG^-_n$ has paths $p:Z_0\to X_0 \pathto C_j \pathto Y$ and $q:Z \upathto C_i \pathto Y$, such that:
\begin{enumerate}
    \item $\calG^-_n$ includes strictly more edges than $\calG^-_{n-1}$, 
    and all added edges are in $p:Z_0 \overset{p}{\to} X_0 \overset{p}{\pathto} C_j$
    \item $C_i,C_j \in \Anc^{\calG_{n-1}}_Y$, i.e.\ paths from $C_i,C_j$ to $Y$ have already been added.
    \item $Z \overset{q}{\upathto} C_i$ is active given $\lceil \bar{\sC}' \cup \bar{\sX}'\rceil \setminus C_i$
    \item $C_i \not \in \Anc^\calG_{C_j} \setminus C_j$
\end{enumerate}
\end{enumerate}

\end{lemma}

\begin{proof}
We will prove the result by induction.
First, we will show that:
(1) holds and $N=0$, or
(2) is satisfied for $\calG^-_0$.
Then we will show that for $n>0$, if (1) or (2) holds for every $n'<n$, then 
(1) holds and $N=n$, or
(2) is satisfied for $\calG^-_n$.
This implies that (2) is true for every $0<n<N$ and (1) is true for $N=n$.

First, consider $n=0$.
If Le 1 is satisfiable for $\bar{\sZ},\bar{\sX}',\bar{\sC}'$, then $N=0$ and 
(1) is immediate, because $\bar{\sZ}$ and $\bar{\sX}'$ have been defined 
to include every edge in $\calG \setminus \calG^-_N$.
Otherwise, by \cref{le:consequences-of-h-cycle}, either 
A) $\bar{\sZ} \not \dsep Y \mid \lceil \bar{\sC}' \cup \bar{\sX}' \rceil$ or B) $\exists C_i,C_j \in \bar{\sC}'$ meeting certain conditions.
For $\calG^-_n$, we have $\bar{\sC}'= \emptyset$, so (A) must be true.
From the definitions of $\bar{\sZ},\bar{\sX}'$, $\calG \setminus \calG^-_n$ contains an edge $Z \to X \in \bar{\sX}'$.
And every decision is an ancestor of $Y$ by nonredundancy \ryan{clarify the nonredundancy assumption}.
So let $p$ be any $Z \to X \pathto Y$.
Let $q$ be any path $Z$ to $Y$, $Z \in \bar{\sZ}$, active given $\lceil \bar{\sC}' \cup \bar{\sX}' \rceil$, thereby satisfying (c).
We have $C_i=C_j=Y$, thereby satisfying (b,d).
We can verify that this satisfies (a-d) \ryan{check/elaborate this last line}

Now, assume that (2) is satisfied for $n' < n$, and we will show that either (1) holds and $n=N$; or (2) is satisfied for $\calG^-_n$.
If Le 1 is satisfiable for $\bar{\sZ},\bar{\sX}',\bar{\sC}'$, then 
$N=n$ and (1) is true as in the $n=0$ case.
Otherwise, by \cref{le:consequences-of-h-cycle}, either 
A) $\bar{\sZ} \not \dsep Y \mid \lceil \bar{\sC}' \cup \bar{\sX}' \rceil$ or B) $\exists C_i,C_j \in \bar{\sC}'$
with 
$\exists Z \in \bar{\sZ}, C_j \in \bar{\sC}' \cap \Desc^\calG_Z, C_i \in \bar{\sC}' \setminus \Anc^\calG_{C_j}$ s.t.
$Z \not \dsep C_i \mid \lceil \bar{\sC}' \cup \sX' \rceil \setminus \{C_i\}$.
If (A), then let $C_i=Y$, choose $p,q$ arbitrarily as in the $n=0$ case, 
and let $C_j$ be the first element of $\bar{\sC'} \cup Y$ in $p$.
Then, we can verify (a-d). \ryan{check/elaborate this}
If (B), then let choose $C_i$ and $C_j$ to match \cref{le:consequences-of-h-cycle}, and (a-d) will be satisfied.
\end{proof}

The intuition is that any edge for which we cannot find paths satisfying (a-e) is a candidate for removal per Le 1. 
Conversely, for any edge that is not a candidate for removal per Le 1, 
there will exist a set of paths $p,q$ satisfying (a-e), and 
for any edges in $p_n,q_n$ that are in $\calG^-_n \setminus \calG^-_0$, 
there will exist a further set of paths $p_{n-1},q_{n-1}$, and so on recursively.

\subsubsection{Example}

To see the kind of paths that can be obtained, we can see the example \cref{fig:stepladder}.

\begin{figure} 
\centering
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv]  {$Z$};
  \node (X) [rv,red,below = 16mm of Z]              {$X$};
  \node (C) [rv, right = 16mm of X]  {$C$};
  \node (Xp) [rv,red,below = 16mm of C]              {$X'$};
  \node (Y) [rv, right = 16mm of Xp]  {$Y$};
  
  \draw[->, very thick, color=gray] (Z) -- (X);
  \draw[->, very thick, color=black] (X) -- (C);
  \draw[->, very thick, color=black] (Z) -- (C);
  \draw[->, very thick, color=black] (C) -- (Xp);
  \draw[->, very thick, color=black] (Xp) -- (Y);
  \draw[->, very thick, color=black] (C) -- (Y);
\end{tikzpicture}
\caption{We want to prove that $Z \to X$ is nonredundant under optimality} \label{fig:stepladder-1}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv]  {$Z$};
  \node (X) [rv,red,below = 16mm of Z]              {$X$};
  \node (C) [rv, right = 16mm of X, line width=0.6mm, dashed]  {$C$};
  \node (Xp) [rv,red,below = 16mm of C,line width=0.6mm]              {$X'$};
  \node (Y) [rv, right = 16mm of Xp]  {$Y$};
  
  \draw[->, very thick, dashed, color=gray] (Z) -- (X);
  \draw[->, very thick, color=black] (X) -- (C);
  \draw[->, very thick, color=black] (Z) -- (C);
  \draw[->, very thick, dashed, color=black] (C) -- (Xp);
  \draw[->, very thick, color=green] (Xp) -- (Y);
  \draw[->, very thick, color=red] (C) -- (Y);
\end{tikzpicture}
\caption{$\calG^0$: shown with solid edges. With $\sX'=X$ and $\sZ=C$, we have a Le1.1 violation, 
highlighted in red.} \label{fig:stepladder-2}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv, line width=0.6mm, dashed]  {$Z$};
  \node (X) [rv,red,below = 16mm of Z,line width=0.6mm]              {$X$};
  \node (C) [rv, right = 16mm of X,line width=0.6mm]  {$C$};
  \node (Xp) [rv,red,below = 16mm of C,line width=0.6mm]              {$X'$};
  \node (Y) [rv, right = 16mm of Xp]  {$Y$};
  
  \draw[->, very thick, dashed, color=gray] (Z) -- (X);
  \draw[->, very thick, color=green] (X) -- (C);
  \draw[->, very thick, color=red] (Z) -- (C);
  \draw[->, very thick, color=black] (C) -- (Xp);
  \draw[->, very thick, color=black] (Xp) -- (Y);
  \draw[->, very thick, color=black] (C) -- (Y);
\end{tikzpicture}
\caption{$\calG^1$: shown with solid edges.
With $\sX'=\{X,X'\},\sZ=Z,\sC'=C$ we have a cycle in the dependency graph, 
which indicates the presence of the paths shown in red and green.} \label{fig:stepladder-3}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv]  {$Z$};
  \node (X) [rv,red,below = 16mm of Z]              {$X$};
  \node (C) [rv, right = 16mm of X]  {$C$};
  \node (Xp) [rv,red,below = 16mm of C]              {$X'$};
  \node (Y) [rv, right = 16mm of Xp]  {$Y$};
  
  \draw[->, very thick, color=gray] (Z) -- (X);
  \draw[->, very thick, color=green] (X) -- (C);
  \draw[->, very thick, color=red] (Z) -- (C);
  \draw[->, very thick, color=black] (C) -- (Xp);
  \draw[->, very thick, color=green] (Xp) -- (Y);
  \draw[->, very thick, color=red] (C) -- (Y);
\end{tikzpicture}
\caption{The red and green paths shown on the original graph.
It is useful for $X$ to observe $Z$ to influence $C$.
In turn, it is useful for $X'$ to observe $C$ to influence $Y$.
} \label{fig:stepladder-4}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv]  {$Z$};
  \node (X) [rv,red,right = 6mm of Z]              {$X$};
  \node (C) [rv, right = 6mm of X]  {$C$};
  \node (Xp) [rv,red,right = 6mm of C]              {$X'$};
  
  \draw[->, very thick] (Z) -- (X);
  %\draw[->, very thick] (Z) to [bend right] (Xp);
  \draw[->, very thick, color=green] (X) -- (C);
  \draw[->, very thick, color=red] (C) to [bend right] (Z);
  \draw[->, very thick] (C) -- (Xp);
  
\end{tikzpicture}
\caption{The dependency graph $\calH$ for $\sX'=\{X,X'\},\sZ=Z,\sC'=C$, which contains the cycle $Z \to X \to C \to Z$.} \label{fig:stepladder-ordering1}
\end{subfigure}
\caption{.} \label{fig:stepladder}
  \end{figure}

In this case, it is not hard to see how we can parameterise these paths in order to exhibit that 
$Z$ is nonredundant under optimality for $X$.

\subsection{A more complicated example}
If, however, $Z$ is a context for other decisions, then it will be more complicated to select an appropriate set of paths.
For example, see \cref{fig:multi-x-step}.
In this case, the theorem gives us some active paths from $Z$ to $C$ to $Y$.
But this has been done with a decision other than $X$.
And then paths are not suitable for parameterising $X$, since $C \in \Pa^\calG_X$.
Concretely, $X$ does not need to observe $Z$ to know about $Y$ along the red paths, because $C$ already provides all such information.
In order to obtain a set of paths that is suitable, we need to choose a different $\sX'$.
In particular, we have showed how $X'$ needs to use the information from $Z$.
So now we can treat $X'$ as a chance node, removing it from $\sX'$.
Then, we have a Thm 1.1 violation, which offers a path $Z \to X' \to Y$.
This gives a more plausible story for why $X$ needs to observe $Z$:
\begin{itemize}
    \item $X$ needs to know $C$ because of the information transmitted by $C \to Y$
    \item $X'$ needs to transmit info from $Z$ because of the information transmitted by $Z \to C \to Y$ (and also $Z \to C \to X \to Y$, in the case that the path from $C$ to $Y$ is not directed).
    \item $X$ needs to transmit info from $Z$ because of the information transmitted by $Z \to X' \to Y$.
\end{itemize}

I haven't yet attempted to prove exactly what paths must exist in cases where $Z$ is a context for multiple decisions.

\begin{figure} 
\centering
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv]  {$Z$};
  \node (Xp) [rv,red,below = 16mm of Z]              {$X'$};
  \node (C) [rv, right = 16mm of Xp,line width=0.6mm,dashed]  {$C$};
  \node (X) [rv,red,below = 16mm of C,,line width=0.6mm]              {$X$};
  \node (Y) [rv, right = 16mm of X]  {$Y$};
  
\draw[->, very thick, color=black] (Z) -- (Xp);
  \draw[->, very thick, color=gray,dashed] (Z) to [bend right=70] (X);
  \draw[->, very thick, color=black] (Xp) -- (C);
  \draw[->, very thick, color=black] (Xp) -- (Y);
  \draw[->, very thick, color=black] (Z) -- (C);
  \draw[->, very thick, color=black,dashed] (C) -- (X);
  \draw[->, very thick, color=green] (X) -- (Y);
  \draw[->, very thick, color=red] (C) -- (Y);
\end{tikzpicture}
\caption{We want to prove that $Z \to X$ is nonredundant under optimality} \label{fig:multi-x-step-1}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv,line width=0.6mm,dashed]  {$Z$};
  \node (Xp) [rv,red,below = 16mm of Z,line width=0.6mm]              {$X'$};
  \node (C) [rv, right = 16mm of Xp,line width=0.6mm]  {$C$};
  \node (X) [rv,red,below = 16mm of C,line width=0.6mm]              {$X$};
  \node (Y) [rv, right = 16mm of X]  {$Y$};
  
\draw[->, very thick, color=black,dashed] (Z) -- (Xp);
  \draw[->, very thick, color=gray,dashed] (Z) to [bend right=70] (X);
  \draw[->, very thick, color=green] (Xp) -- (C);
  \draw[->, very thick, color=black] (Xp) -- (Y);
  \draw[->, very thick, color=red] (Z) -- (C);
  \draw[->, very thick, color=black] (C) -- (X);
  \draw[->, very thick, color=black] (X) -- (Y);
  \draw[->, very thick, color=black] (C) -- (Y);
\end{tikzpicture}
\caption{When we have $\sX'=\{X,X'\},\sC'=C,\sZ=Z\}$} \label{fig:multi-x-step-2}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv,line width=0.6mm,dashed]  {$Z$};
  \node (Xp) [rv,red,below = 16mm of Z]              {$X'$};
  \node (C) [rv, right = 16mm of Xp,line width=0.6mm]  {$C$};
  \node (X) [rv,red,below = 16mm of C,line width=0.6mm]              {$X$};
  \node (Y) [rv, right = 16mm of X]  {$Y$};
  
\draw[->, very thick, color=red] (Z) -- (Xp);
  \draw[->, very thick, color=gray] (Z) to [bend right=70] (X);
  \draw[->, very thick, color=black] (Xp) -- (C);
  \draw[->, very thick, color=red] (Xp) -- (Y);
  \draw[->, very thick, color=black] (Z) -- (C);
  \draw[->, very thick, color=black] (C) -- (X);
  \draw[->, very thick, color=green] (X) -- (Y);
  \draw[->, very thick, color=black] (C) -- (Y);
\end{tikzpicture}
\caption{When we remove $X'$ from $\sX'$, Le1.1 is violated (red path)} \label{fig:multi-x-step-3}
\end{subfigure}
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (Z) [rv]  {$Z$};
  \node (X) [rv,red,right = 6mm of Z]              {$X$};
  \node (C) [rv, right = 6mm of X]  {$C$};
  \node (Xp) [rv,red,right = 6mm of C]              {$X'$};
  
  \draw[->, very thick] (Z) -- (X);
  \draw[->, very thick] (Z) to [bend right] (Xp);
  \draw[->, very thick, color=green] (X) -- (C);
  \draw[->, very thick, color=red] (C) to [bend right] (Z);
  \draw[->, very thick] (C) -- (Xp);
  
\end{tikzpicture}
\caption{The dependency graph $\calH$ for $\sX'=\{X,X'\},\sC'=C,\sZ=Z$, which contains the cycle $Z \to X \to C \to Z$.} \label{fig:stepladder-ordering2}
\end{subfigure}
\caption{.}\label{fig:multi-x-step}
\end{figure}





%ryan: ideas about how to incorporate the Thm 2 condition into this



%Now, we show what this implies for a specific edge-accumulation procedure.
%Formally, suppose we're identifying which edges are nonredundant under optimality (NRO) in a graph $\calG$ induced by a scope $\calS = \langle X,C_X \rangle_{X \in \sX}$.

%\begin{definition}
%Let $\calG^-_0$ be $\calG$ but without every edge $C \to X$ that is incoming to a decision $X \in \sX$.
%Then, obtain $\calG^-_i$ from $\calG^-_{i-1}$ by adding any edge $C \to X$
%such that there exist paths 
%$p:X \pathto Y$ in $\calG$
%and $q:C \upathto Y$ in $\calG^-_{i-1}$
%where $q$ is active in $\calG^-_{i-1}$ given $C_{\sXnew} \setminus \{C\}$, 
%where $\sXnew = X \cup \{X' \in \sX \mid V \to X' \in p \text{ and } V \to X' \not \in \calG^-_{i-1}\}$.
%When no more edges may be added, call resulting graph is $\calG^-$.
%\end{definition}

==> sections/old/y-tricky-graph.tex <==
\section{New tricky graph}



\begin{figure} \centering
\begin{subfigure}[b]{0.42\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (1) [rv,red,label=below:$\in \mathbb{B}^2$]              {$X^1$};
  \node (Z) [rv, above = 2.8cm of 1,label=$z \sim \mathbb{B}$]  {$Z$};
  \node (Y) [rv, right=2.2cm of 1,label=below:{$y=\llbracket f[x^1[0]]=x^1[1]\rrbracket$}] {$Y$};
  \node (F) [rv, above = 2.8cm of Y,label=above:$f \sim \mathbb{B}^2$]  {$F$};
  \node (3) [rv,red, above right= 0.6cm and 0.8cm of 1,label=right:$\in \mathbb{B}$] {$X^2$};
  \node (W) [rv, above = 0.6cm of 3,label={$w=f[z]$}]  {$W$}; %

  \draw[->, very thick, color=gray] (Z) -- (1);
  \draw[->, very thick, color=blue] (Z) -- (W);
  \draw[->, very thick, color=blue] (F) -- (W);
  \draw[->, very thick, color=blue] (F) -- (Y);
  \draw[->, very thick, color=blue] (W) -- (3);
  \draw[->, very thick, color=blue] (Z) -- (3);
  \draw[->, very thick, color=blue] (1) -- (Y);
  \draw[->, very thick, color=blue] (3) -- (1);
\end{tikzpicture}
\caption{
The given parameterisation shows that $Z$ is nonredundant.
} 
\label{fig:causal-graph-3}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (1) [rv,red,label=below:{$=01$}]              {$X^1$};
  \node (Z) [rv, above = 2.8cm of 1,label={$z =0$}]  {$Z$};
  \node (Y) [rv, right=2.2cm of 1,label=below:{$y=\llbracket 1=1 \rrbracket=1$}] {$Y$};
  \node (F) [rv, above = 2.8cm of Y,label=above:{$f=10$}]  {$F$};
  \node (3) [rv,red, above right= 0.6cm and 0.8cm of 1,label=right:{$=1$}] {$X^2$};
  \node (W) [rv, above = 0.6cm of 3,label={$w=1$}]  {$W$}; %

  \draw[->, very thick, color=gray] (Z) -- (1);
  \draw[->, very thick, color=blue] (Z) -- (W);
  \draw[->, very thick, color=blue] (F) -- (W);
  \draw[->, very thick, color=blue] (F) -- (Y);
  \draw[->, very thick, color=blue] (W) -- (3);
  \draw[->, very thick, color=blue] (Z) -- (3);
  \draw[->, very thick, color=blue] (1) -- (Y);
  \draw[->, very thick, color=blue] (3) -- (1);
\end{tikzpicture}
\caption{
A sample from the graph to the left
} 
\label{fig:causal-graph-4}
\end{subfigure}
\caption{Another tricky-to-parameterise graph (left) and a sample from the parameterisation (right)}
\end{figure}

I found a new interesting graph: \cref{fig:causal-graph-3}.
Sanghack's comments provide a decent summary: \emph{Does $X^1$ need to listen to $Z$ how $X^2$ best reconstructs $F$? If we do not restrict the dimensionality of $X^2$, then $X^2$ will reconstruct $F$ as much as possible and pass the information to $X^1$. But let's assume that $X^2$ is just binary and $Z$ be high-dimensional. $X^1$ may use some information from $Z$.}

We can parameterise the graph to exhibit that $Z$ is nonredundant, roughly as Sanghack suggests --- this is shown.
But this places a constraint on our solution space: for decisions like $X^2$ that are in $\sX \cap \Ch_Z \cap \Anc_{X^1}$, 
we need to take care not to give them any ``spare bits'' that they can use to transmit information about $Z$.

A second consideration is that we need to make sure any recursive parameterisation scheme bottoms out.
In particular, if we're trying to exhibit that $Z$ is nonredundant for $X^1$ by showing that $Z$ is nonredundant for $X^2$, 
then it's quite unclear how to make such a recursion bottom out, given that $X^2$ is an ancestor of $X^1$.

Based on these considerations, I proposed a slightly modified scheme.

\section{New scheme [rough notes]}
The new scheme is essentially to generalise the approach of $\cref{fig:causal-graph-3}$ to multiple $W^i$ nodes.

Assume that we want to exhibit that $Z^0$ is nonredundant for $X^0$.
Let $SP(A,B)$ denote the shortest directed path from $A$ to $B \in \Desc_B$.
Since Le1.1 is violated, we have paths:
\begin{itemize}
\item Let $p^0=SP(X^0,Y)$. Write $p^0$ as $X^0 \pathto Z^1 \to X^1 \to \ldots \to Z^K\to X^K \pathto Y$, 
and then let each $p^k=SP(X^k,Y)$ be a segment of $p^0$.
\ryan{We assume for now that each $Z^k$ is not in $\sX$, i.e.\ $Z^k \neq X^{k-1}$ --- we will later have to relax this assumption.}
\item Let $q^k$ be any $Z^k \upathto Y$ that is active given $\lceil \sC \cup \sX \rceil$ (the path is chosen arbitrarily),
\item Let $\{r^k_i\}_{i \leq k}=SP(W_i,Y)$ for each collider in $q^k$.
\end{itemize}

Also, define some nodes in each $q^k$:
\begin{itemize}
\item Let the forks be $\{F^i\}_{1\leq i \leq I}$, counting $Z^k$ as a ``fork'' $Z^k=F^1$ iff $q^k$ is front-door.
\item Let the colliders be $\{W^i\}_{1\leq i < I}$.
\end{itemize}

The aim of the scheme will be to have $\mathbb{E}[Y]=K$,
but that if the edge $Z^0 \to X^0$ is removed, then $\mathbb{E}[Y]<K$ under every policy.

We assign the functions:
\begin{itemize}
\item each fork in $q^k$ (excluding $Z^k$) is a uniform random bitstring $F^i \sim (\text{Bernoulli}(\frac{1}{2})_j)_{j \in 1,2,\ldots,(k+i)^2}$
\item write each collider $W^i$ in $q^k$ with $W^i=V^n$ as $V^{n-1} \to V^n \gets V^{n+1}$ and has function $V^n=V^{n+1}[V^{n-1}]$
\item each chain in $p^k,q^k$ or $r^k$ is equal to its parent within that path
\item each decision $X^k=Z^k$
\item Let $\pa^p_N$ denote the parent of $N$ along path $p$. Then, $Z^k$ is defined as:
\begin{itemize}
    \item if $q^k$ is frontdoor, $Z^k=(\text{Bernoulli}(\frac{1}{2})_k)_{k \in 1,2,\ldots 2^k}[\pa^{p^0}_{Z^k}]$ for $k>0$ and $Z^0=(\text{Bernoulli}(\frac{1}{2}))$ for $k=0$.
\item Otherwise, $Z^k=\pa^{q^k}_{Z^k}[\pa^{p^0}_{Z^k}]$ for $k>0$ and $Z^k=\pa^{q^k}$ for $k=0$.
\end{itemize}
\item $Y= \sum_k Y^k$ where 
$Y^k = 
\begin{cases}
1 & \text{ if } \exists \{s^i\in \mathbb{B}^{2^(k+i)}\}_{i \in 1,2,\ldots I}, 
\text{ s.t.\ } s^I=F^I,s^1=\pa^{p^0}_Y \text{ and each } s^i[s^{i-1}]=\pa^{r^i}_Y \\
0 & \text{otherwise}
\end{cases}
$
\end{itemize}



If any node lies in multiple paths, let its function be the cross-product of the respective functions.
\ryan{I haven't yet made this clear at all, but each node $V$ in $p^k$ also lies in $p^{Z^{k-1},X^{k-1}}$, and so on, so it carries $k$ bits.}
Since any $X^k$ is downstream of $X^{k-1}$, the recursion bottoms out.

Intuitively, the decision at $X^0$ is tasked with describing (along with a decision that passes info from each $W^i$)
what values of $f^I$ are possible, given what these decisions know.
They do not know $F^I$, but they do know $W^I$, which is one of its digits.
They do not know the exact index $F^{I-1}$ of this digit, but they know $W^{I-1}$, which is one of the digits of the index.
And so on...
The decisions will indicate that some $2^k$ sequences are not possible at $F^I$.
In the non-intervened graph, the decisiosn will accurately represent exactly what is known, and obtain $Y=k$.
However, if the context $Z^0$ is removed from $X^0$, we should be able to prove that $\mathbb{E}[Y]<k$ is impossible.


The logic of this approach is that we have parameterised each $r_i^{Z,X}$ to have exactly the number of bits required to transmit the 
information of each $W^i$ to $Y$.
To achieve $\mathbb{E}[Y^k]=1$, we require $X^k=Z^k$.
If $X^k=Z^k$, then to achieve 
$\mathbb{E}[Y^{k-1}]=1$, we will need $X^{k-1}=Z^{k-1}$ too, 
and so on to $X^{0}=Z^{0}$
If we achieve $X^{0}=Z^{0}$ without using the edge $Z^0 \to X^0$, this will have to use up a bit from elsewhere in the graph.
But this would prevent us from properly transmitting the bit along some $r^i$, which would also mean that $\mathbb{E}[Y^k]<1$.
So the context $Z^0$ is required at $X^0$ for optimal performance.

\begin{figure}\centering
\begin{tikzpicture}[rv/.style={circle, draw, thick, minimum size=6mm, inner sep=0.8mm}, node distance=15mm, >=stealth]
  \node (1) [rv,red,label=below:{}]              {$X^0$};
  \node (Z) [rv, above = 2.8cm of 1,label={$f\sim \text{Bernoulli}$}]  {$Z^0$};
  \node (Y) [rv, right=4.6cm of 1,label=below:{}] {$Y$};
  \node (F2) [rv, above = 2.8cm of Y,label=above:{$f\sim \text{Bernoulli}^4$}]  {$F$};
  \node (X2) [rv, red, above right= 0.4cm and 0.8cm of 1,label=right:{$=w^1$}] {$X^1$};
  \node (W1) [rv, above = 0.6cm of X2,label={}]  {$W^1$}; %
  \node (F1) [rv, above right= 0.6cm and 0.8cm of W1,label=above:{$f\sim \text{Bernoulli}^2$}] {$F^1$};
  \node (X3) [rv,red, right= 1.8cm of X2,label=right:{$=w^2$}] {$X^2$};
  \node (W2) [rv, above = 0.6cm of X3,label={}]  {$W^2 $}; %


  \draw[->, very thick, color=gray] (Z) -- (1);
  \draw[->, very thick, color=blue] (Z) -- (W1);
  \draw[->, very thick, color=blue] (F2) -- (W2);
  \draw[->, very thick, color=blue] (F2) -- (Y);
  \draw[->, very thick, color=blue] (W2) -- (X3);
  \draw[->, very thick, color=blue] (F1) -- (W1);
  \draw[->, very thick, color=blue] (F1) -- (W2);
  \draw[->, very thick, color=blue] (X3) -- (Y);
  \draw[->, very thick, color=blue] (W1) -- (X2);
  \draw[->, very thick, color=blue] (Z) -- (X2);
  \draw[->, very thick, color=blue] (1) -- (Y);
  \draw[->, very thick, color=blue] (X2) -- (1);
\end{tikzpicture}
\caption{
.
} 
\label{fig:causal-graph-4}
\end{figure}

\ryan{
Currently, I'm thinking about how to prove that if one bit is ``wrong'' at $Y$, then 
there will always exist a value of $F^I$ such that $Y=0$.
I'm thinking that for each bitstring $(b_1,...,b_I)$ that is offered to $Y$, it means that $I^2$
possible values of $F^j$ are dis-allowed.
My current hope is that I could prove by induction (over bitstring length) that the set of $I^2$ dis-allowed 
$F^j$ values differs for any distinct bitstring, 
so whatever bitstring was offered, there exists a bitstring that was disallowed, but that can actually 
happen, leading to $U=0$.
}

\ryan{It would probably be possible to use XORs instead of indexing. XORs are cleaner/easier. But they has a few disadvantages. One is that information passed down from the $W^i$ nodes can be compressed whenever $W^i$ and $W^j$ are observed. So it's trickier to ensure that spare bits cannot be freed up, in order to give an alternate way for $X^0$ to know $Z^0$. A second disadvantage is that it would require two approaches: both indexing (to ensure that $X^k$ passes on information from $Z^k)$ and XORs, whereas this approach is purer, in that it only involves indexing.}

\Ryan{My current uncertainties are:
- how exactly do I prove that whenever a ``wrong'' bit is selected, then performance can be penalised?
%- should I be reverting back to the XOR approach
- how exactly will this extend to cases where some $Z^k$ is a decision
- how exactly will this extend to cases where Le 1.1 is satisfiable but Le1.1-1.3 is not? (I think I can use my lemmas about the existence of paths $q^k$, but I'll need to check whether any changes are needed.
- am I reinventing the wheel somehow? e.g.\ does there exist a known distribution with properties like this? An encryption algorithm that behaves in this way?
- can I tweak the setup so there's a simple mapping from a bitstring $(b_j)_j$ to the set of allowed $f_j$ values?
}


\Ryan{Probably switch to subscripts everywhere, if I'm using powers.}
\Ryan{the parents notation is OK.}
\Ryan{$q^k$: two colliders, what to do about this?}
%$\mathfrak{ABCDEFGHIJKLMONPQRSTUVWXYZ}$

==> sections/old/z-earler-lemmas.tex <==
\section{Earlier lemma statements}
\Ryan{Add the simplification of Lemma 1.}

%\begin{lemma}[Le1.1 and 1.3 satisfiable with unitary Z] 
%If $\exists \mathbf{Z} \ni Z, \sX', \sC', \prec, \sU = \emptyset$ that satisfies Le1.1 $\exists \mathbf{Z} = {Z}, \sX', \sC', \prec, \sU = \emptyset$ that satisfies Le1.1 and Le1.3  
%\end{lemma}
%\ryan{should generalise this to no-longer require $\sU=\emptyset$.}
%\ryan{must add proof}

\begin{lemma}[maximal conditioning set d separates X from Y(i.e. satisfies Le1.1)] \label{le:max-cond-satisfies-1.1}
    Lemma: let $\mathbf{X} \subseteq Anc(Y)$ and $\mathbf{C} = \bigcup_{x \in X} \sC_X \backslash Z$. 
    If $\exists \mathbf{C'} \subseteq \mathbf{C}$, $\exists \mathbf{X'} \subseteq \mathbf{X} : Z \perp Y \mid \mathbf{C'} \cup \mathbf{X'}$, then $Z \perp Y \mid \mathbf{C} \cup \mathbf{X}$
\end{lemma}
\ryan{Maybe should be $\Pi$ rather than $Z$.}
\ryan{must add proof}


First, I state a generally useful Lemma:
\begin{lemma}[active path to descendant of all conditioning variables is active given any subset of conditioning set] \label{le:active-to-ancestors-preserved-subset}
If $\sA \not \dsep \sB \mid \sW$ and $\sW \subseteq \Anc_{\sB}$
then $\sA \not \dsep \sB \mid \sW'$ for any $\sW' \subseteq \sW$.
\end{lemma}

\begin{proof}
By $\sA \not \dsep \sB \mid \sW$, there exists a path $q:\sA \upathto \sB$, active given $\sW$.
If every collider in $q$ is in $\Anc_{\sW'}$, then we already know that every non-collider is not in $\sW' \subseteq \sW$, 
so $q$ is active given $\sW'$.
Otherwise, let $C$ be the first collider in $q$ that is not in $\Anc_{\sW'}$. 
Then $q':A \overset{q}\upathto C \pathto B$ is active given $\sW'$:
the first segment is active by the same argument as the previous case, and
the second segment (including $C$) is active because $C \not \in \Anc_{\sW'}$.
\end{proof}

==> sections/old/z-old-h-graph.tex <==
\section{Proof elements}
Le1 says that $Z$ is redundant under optimality if we can choose an ordering $\prec, \sC', \sZ\ni Z$
that satisfies criteria Le1.1-1.3. (And $\sU$, but we tentatively assume that $\sU=\emptyset$.)
We are assuming that Le1.1-1.3 are not satisfiable, and 
we want to construct a set of paths, that exhibits why Le1.1-1.3 is unsatisfiable.
Ultimately, we will use this set of paths to choose functions $f$ and probability distributions $P$ to exhibit why an edge $Z \to D$ is nonredundant under optimality (the completeness result).
Our strategy for obtaining such a set of paths is to choose some $\sC'_0,\sZ_0$ then compute a graph $\calH'_i$. 
%so that letting $\prec$ be any topological order over $\calH_i$ will satisfy Le1.1-1.3.
%Since Le1.1-1.3 is unsatisfiable, we will always be able to find a cycle.
%So we note that down, modify $\sC'_i,\sZ_i,\calH'_i$ to obtain another cycle, and repeat the process until we obtain a cycle that contains $Y$.
To compute the graph $\calH'_i$, we add an edge $A \to B$ where
Le1.1-1.3 requires $A \prec B$ for \emph{any} ordering $\prec$ consistent with the edges already present, 
and repeat this process until reaching the fixed point $\calH'_i$.
We will prove that any topological ordering $\prec$ on $\calH'_i$ will satisfy Le1.1-1.3.
Since Le1.1-1.3 is unsatisfiable, this means there must be a cycle in $\prec$.
We then use this to obtain some paths in $\calH'_i$ (and hence in $\calG$).
Then we obtain a modified $\sC'_{i+1},\sZ_i,\calH'_i$ and repeat the process.

To find an edge $A \to B$ that is in ordering $\prec$, we will require there to be a walk that is d-connected given 
two different sets of nodes.

\begin{definition}[Active walk]
A walk $w:A\upathto B$ is active given $\sC$ if every collider in $\sw$ is in $\sC$ and every non-collider is not.
\end{definition}

\begin{lemma}[Ancestors of closure] \label{le:ancestors-of-closure}
If $V \in \lceil \sV \rceil$ and $A \in \Anc^\calG(V) \setminus \lceil \sV \rceil$ then $A \in \Anc^\calG(\sV)$
\end{lemma}
\begin{proof}
We will prove the contrapositive. 
We assume that $A \not \in \Anc^\calG (\sV)$
and 
$A \in \Anc^\calG(V) \setminus \lceil \sV \rceil$.
Then, we will prove that $V \not \in \lceil \sV \rceil$.
Choose any path $p:A = N^1 \to N^2 \to ... N^n = V$.
Then, every $N^i$ is not in $\sV$ by assumption.
Moreover, $A=N^1 \not \in \lceil \sV \rceil$,
and $N^{i-1} \not \in \lceil \sV \rceil \implies N^i \not \in \lceil \sV \rceil$
by the definition of $\lceil \cdot \rceil$.
So by induction, $V=N^n \not \in \lceil \sV \rceil$, 
proving the result by contrapositive.
\end{proof}


\begin{definition}[Ordering graph ($\calH$)]
Let $\calG$ be a causal graph containing whose vertices include the following disjoint sets: $\sC',\sX,\sZ,\{Y\}$.
Then, the \emph{partial ordering graph} is the graph $\calH$ with vertices $\sC' \cup \sX' \cup Z \cup \{Y\}$, 
containing an edge $A \to B$ if and only if: (i) $A \in$ Pa$^\calG_B$ and $B\in \sX'$, or ii) $A\in \sX'$ and $B \in$ Desc$^\calG_A$.

The \emph{full ordering graph} $\calH'$ is obtained from the partial ordering graph by $\calH'=h(\calH, \calG)$
where
$$
h(\calH) = 
\begin{cases}
(\sV_{\bar\calH},\sE_{\bar\calH} \cup (C \to Z)) & \text{if $\calG$ contains a walk $w:Z\upathto C, C \in \sC', Z \in \sZ \setminus \Anc^{\calH}_C$, active } \\ 
 &\text{given $\lceil (\sC' \cup \sX') \cap \Anc^\calH_{Z \cup C} \rceil$ and active given $\lceil \sC' \cup \sX' \rceil$.} \\
\calH	& \text{otherwise}.
\end{cases}
$$
\end{definition}
(When multiple $C \in \sC, Z\in\sZ$ satisfy the condition, we choose such a $C,Z$ arbitrarily.)
\ryan{Should I change this to remove the endpoints $Z$ and $C$ from the conditioning set(s)?}

Firstly, we will establish that $\calH'$ encodes all of the requirements of Le1.1-1.3.

\begin{lemma} \label{le:dsep-given-ancestors}
Let $\calH'$ be the ordering graph for any $\calG,\sX',\sC',\sZ,Y$.
Then, $\forall Z \in \sZ, C \in ( \sC \cup \{Y\}) \setminus \Anc^{\calH^*}_{Z}, C \perp Z \mid \lceil ( \sC' \cup \sZ) \cap \Anc^{\calH'}_{Z\cup C} \rceil$
 \end{lemma}

Assume that $\exists Z \in \sZ, C \in ( \sC \cup \{Y\}) \setminus \Anc^{\calH'}_{Z}, C \not \perp Z \mid \lceil ( \sC' \cup \sZ) \cap \Anc^{\calH'}_{Z\cup C} \rceil$, 
and then we will prove a contradiction.
Choose any $Z \in \sZ, C \in ( \sC \cup \{Y\}) \setminus \Anc^{\calH'}_{Z}$ with a walk $w:Z \upathto C$, active given $\sW:=\lceil (\sC' \cup \sZ) \cap \Anc^{\calH'}_{Z\cup C} \rceil$.
Since $C \not \in \Anc^{\calH'}_Z$, the ordering graph $\calH'$ does not contain $C \to Z$, 
so by the definition of $h$, the walk $w$ must be blocked by $C \perp Z \mid \lceil (\sC' \cup \sX') \rceil$.
Since $\sW \subseteq \lceil (\sC' \cup \sX')\rceil$, 
%the walk $w$ cannot be blocked by $\lceil (\sC' \cup \sX')\rceil$ at a collider, so 
$w$ must be blocked at a non-collider in $\lceil (\sC' \cup \sX') \rceil \setminus \sW$.
So let $V$ be the non-collider nearest to $Z$ in $w$ such that $V \in \lceil (\sC' \cup \sX') \rceil \setminus \sW$.

Then, either $V \in \sC'$ or $V \not \in \sC'$.
If $V \in \sC'$, then 
the segment $Z \overset{w}{\upathto} V $ is
active given $\sW$
and active given $(\sC' \cup \sX')$,
so by the definition of $h$, the edge $\sC' \ni V \rightarrow Z$ is in $\calH'$, and $V \in \sW$, yielding a contradiction. 

So instead, suppose that $V \not \in \sC'$.
Then, the closure property $\lceil \cdot \rceil$, by its definition, can only add decisions to any set, i.e.\ $\sW \subseteq (\sC' \cup \sX') \cup \sX)$, so $V$ must be a decision ($V\in \sX$). 
%Together with the fact that $V \not \in \Anc^{\calH'}_{Z \cup C}$ (from the definition of $h$),
%this tells us that $V \not \in \Anc^{\calG}_{Z\cup C}$.
Moreover, we assumed that $V$ was a non-collider in $w$, 
so $w$ must contain at least one path $V \pathto N$ where $N$ is a collider
or an endpoint.
The endpoints $\{Z,C\}$ are in clearly in 
$\Anc^{\calH'}_{Z \cup C}$.
Moreover, the colliders are in
$\sW=\lceil (\sX' \cup \sC') \cap \Anc^{\calH'}_{Z \cup C} \rceil$
by activeness of $h$, 
while $V$ is not.
It follows from \cref{le:ancestors-of-closure} that 
\begin{align*}
V &\in \Anc^\calG ((\sX' \cup \sC') \cap \Anc^{\calH'}_{Z \cup C}) & \\
& \in \Anc^\calG (\Anc^{\calH'}_{Z \cup C}) & (intersection) \\
& \in \Anc^{\calH'} (\Anc^{\calH'}_{Z \cup C}) & (V \in \sX') \\
%& \in \Anc^{\calH'}({Z \cup C}) & \\
& \in \lceil (\sC' \cup \sZ) \cap \Anc^{\calH'}_{Z \cup C} \rceil & (V \in \sX')
\end{align*}
This contradicts the assumption that $V \not \in \sW$, showing the result.

%Then there must be a walk $w$ from $Z$ to $C$ active given $ \lceil(\sC' \cup \sX') \cap \Anc^{\calH'}_{Z\cup C} \rceil $ but blocked given $ \lceil (\sC' \cup \sX') \rceil $.
%Any such walk must contain a non-collider in $\sW=\lceil (\sC' \cup \sX') \rceil \setminus \sW $ (by the definition of an of active walk \& $\lceil (\sC' \cup \sX') \cap (\Anc^{\calH'}_{Z\cup C} )  \rceil \subseteq \lceil (\sC' \cup \sX') \rceil$).
%
%Choose such a walk $w:Z\upathto C$ arbitrarily, and let $V$ be the non-collider in $\sW$ nearest to $Z$.
%
%Then, either $V \in \sC'$ or $V \not \in \sC'$.
%If $V \in \sC'$, then 
%the segment $Z \overset{w}{\upathto} V $ is
%active given $\lceil( \sC' \cup \sX') \cap \Anc^{\calH'}_{Z\cup C} \rceil $
%and active given $( \sC' \cup \sX')$,
%so by the definition of $h$, the edge $V \rightarrow Z \in \sC'$ must be in $\calH^*$, yielding a contradiction. 
%
%So instead, suppose that $V \not \in \sC'$.
%Then, the closure property, by its definition, can only add decisions to any set, i.e.\ $\lceil (\sC' \cup \sX')\cap \Anc^{\calH'}_{Z \cup C}\rceil \subseteq (\sC' \cup \sX') \cup \sX)$, so $V$ must be a decision ($V\in \sX$). 
%Together with the fact that $V \not \in \Anc^{\calH'}_{Z \cup C}$ (from the definition of $h$),
%this tells us that $V \not \in \Anc^{\calG}_{Z\cup C}$.
%Moreover, we assumed that $V$ was a non-collider in $w$, 
%so $w$ must contain at least one path $V \pathto N$ where $N$ is a collider.
%
%
%So...........
%By assumption, $N \in \lceil( \sC' \cup \sX') \cap \Anc^{\calH'}_{Z\cup C} \rceil$. Also $N \in \Desc^{\calG}V$.
%
%This implies that $V \in \lceil (\sC' \cup \sX') \cap \Anc^{\calH'}_{Z\cup C} \rceil$ (because $N \in \lceil \sN \rceil, V \in Anc_{N} \Rightarrow V \in \lceil \sN \rceil$) by \cref{still-need-to-prove this}), yielding a contradiction.








\begin{lemma}[Topological ordering implies Le1.2 not violated] \label{le:dsep-given-ordering}
Let $\calH'$ be the ordering graph for any $\calG,\sX',\sC',\sZ,Y$, and $\prec$ be any topological ordering over $\calH'$.
Then, $\sZ_{\prec C} \dsep_\calG C \mid \lceil(\sX' \cup \sC')_{\prec C}\rceil$ for all $C \in (\sC' \cup \{Y\})$.
\end{lemma}
\begin{proof}
%We will assume that $\sZ_{\prec C} \not \dsep_\calG C \mid \lceil(\sX' \cup \sC')_{\prec C}\rceil$ 
Assume $\sZ_{\prec C} \not \dsep_\calG C \mid \lceil(\sX' \cup \sC')_{\prec C}\rceil$ and then we will prove a contradiction.
Choose any $C \in \sC' \cup \{Y\}, Z \in \sZ_{\prec C}$ with a walk $w: Z\upathto C$, active given $\lceil (\sX' \cup \sC')_{\prec C}\rceil$.

By \cref{le:dsep-given-ancestors}, $w$ is blocked given $\sW := \lceil (\sX' \cup \sC') \cap \Anc^{\calH'}_{C \cup Z} \rceil$.
So let $C^1$ be the node furthest from $Z$ in $w$ such that $C^1 \in \sC' \cup \{Z, Y \}$ and $Z \overset{w}{\upathto} C^1$ is active given $\sW$, 
and let $C^2$ be the node nearest to $Z$ in $w$ such that $C^2 \in \sC' \cup \{ Y \}$ and $Z \overset{w}{\upathto} C^2$ is blocked given $\sW$.

%Let $C'$ be the node nearest $Z$ in $w$ s.t. $C' \in \sC' \cup \{ Y \}$ 
%and the (shortest) walk  $w':Z\overset{w}{\upathto}C'$ is blocked given $\lceil (\sX' \cup \sC') \cap \Anc^{\calH'}_{C \cup Z} \rceil$ (which must exist since $C'$ meets these conditions by \cref{le:dsep-given-ancestors}).
%Let $V$ be the node nearest $C'$ in $w'$ s.t. $C \in Z \cup \sC' \cup \{ Y \}$ and the (shortest) walk $w'':Z\overset{w'}{\upathto}C$ is active given $\lceil (\sX' \cup \sC') \cap \Anc^{\calH'}_{C \cup Z} \rceil$.

%\ryan{NB. hopefully I don't need walks in the end...}

We now know of the segment $w':C^1 \overset{w}{\upathto} C^2$ that:

\noindent\begin{tabular*}{\textwidth}{@{}l@{\extracolsep{\fill}}r@{}}
(1) it is blocked given $\sW$ & (defs of $C^1,C^2$) \\
(2) it is active given $\lceil (\sX' \cup \sC')_{\prec C} \rceil$ & (because $w'$ is a segment of $w$) \\
(3) does not contain $\sC' \cup \{Y\}$ except at its endpoints & (defs of $C^1,C^2$) \\
(4) every collider is in $\lceil (\sX' \cup \sC') \rceil \backslash \sC'$ &(from 2, 3) \\
(5) every collider is in $\sX$ &(from 4 \& definition of $\lceil \cdot \rceil$) \\
\end{tabular*}

So write $w'$ as $C^1 \upathto X^{1} \leftarrow Z^{1}\upathto X^{n} \leftarrow Z^n \upathto C^2$ (from 3, \& the fact that every parent of X is in $\sZ \cup \sC'$). 
Then $C^2 \not \dsep Z^n \mid \sW$ (from 2,5).
So $C^2 \in \Pa^{\calH'}_{Z^{n}}$ (by def of $\calH$).
Moreover, $Z^{n} \in \Pa^{\calH'}_{X^{n}}$ (by def of $\calH$).
Hence $C^2 \in \Anc^{\calH'}_{X^{n}}$.

If $C^2 \in \Anc^{\calH'}_{X^{n}}$, then $C^2 \in \Anc^{\calH'}_{X^{n}}$ by the same argument.
By induction, $C^2 \not \dsep Z \mid \sW$.

But this contradicts the assumption that there could exist some segment $w'$, blocked given $\sW$, thereby proving the result.

\end{proof}




%\robin{Should be able to use that if there is any m-connecting path for $A$ and $B$ given $C$, then there is one contained in the ancestors of $A \cup B \cup C$.  Hence, the topological order should solve the problem?  Might have to be careful about the closure though.}
%\ryan{I don't know if I follow how this would work. (Note that the $\Anc$ in $h$ is with respect to the ordering graph, i.e.\ $\Anc^{\calH}$.)}

\begin{lemma}[Topological ordering satisfies Le1.1-1.3] \label{le:top-ordering-satisfies-le1}
Let $\sC'$ and $\sZ$ satisfy Le1.1, and $\sU=\emptyset$.
Let $\calH'$ be the ordering graph for $(\calG,\sC',\sZ,\sU)$.
Then, for any topological ordering $\prec$ on $\calH'$, $\sC',\sZ,\sU,\prec$ satisfies Le1.1-Le1.3
\end{lemma}
\begin{proof}
If $\prec$ is topological on $\calH'$, it satisfies Le1.1-Le1.2 by \cref{le:dsep-given-ordering}.\ryan{check that this exactly matches what we prove above}
Moreover, a topological ordering on $\calH'$ clearly satisfies Le1.3, proving the result.
\end{proof}

This can also be understood in the contrapositive direction:
if Le1.1-1.3 are not satisfiable, then $\calH'$ must contain a cycle, 
a fact that we will use to prove the existence of certain structures in $\calG$.

==> sections/old/z-old-simplifying-thm2.tex <==
\section{Simplifying Le 1}
\begin{lemma} \label{le:simplified-le1}
If for some $C$, we have
$C \dsep^\calG \sZ_{\prec C},\sU' \mid \lceil (\sX' \cup \sC')_{\prec C} \rceil$ (A)
and Le 1.3 holds, 
then
$C \dsep^\calG \spi_{\sX'_{\prec C}},\sZ_{\prec C},\sU' \mid \lceil (\sX' \cup \sC')_{\prec C} \rceil$
\end{lemma}
\begin{proof}
We will prove that for any $C \in \sC',X \in \sX'_{\prec C}$, we have $\spi_X \dsep C \mid \lceil (\sX' \cup \sC')_{\prec C} \rceil$.
Since $X$ is in the conditioning set,
Since $X$ is the only child of $\spi_X$, any active path $p$ to $\sPi_X$
would have to pass through $X$. 
And we know that $X \prec C$, so $X$ is in the conditioning set, 
so any $p$ cannot have $X$ as a collider.
By Le 1.3, any parent $C \in C_X \cap (\sC' \cup \sX')$
has $V \prec C$ so must also block $p$.
Since $\sZ$ subsumes, $\sC_{\sX'} \setminus (\sC' \cup \sX')$, 
so the only remaining possibility for $p$ would be a path $\pi_X \to X \gets Z \upathto C$.
But we have already assumed that $Z$ is d-separated from $C$.
So no active path $p$ can exist, and the result follows.
\end{proof}

Thus we can remove $\spi_{\sX'_{\prec C}}$ from the Lemma 1.2 condition.

\section{Simplifying Thm 2}
It seems to me that theorem 2 can be stated more simply.

%\begin{conjecture}
%$\forall X \in \sX', \fix(\sC_X \setminus \sZ) \supseteq \sC_X$ where $\fix(\sT)=\sT$ if $\sT=\hat{\sT}$ aind $\fix(\hat{\sT})$ otherwise, 
%where $\hat{\sT}=\lceil \sT\rceil \cup \{Z \in \sZ:\exists \sV_Z \subseteq(\sV'_{\prec Z} \cup \sU') \cap \lceil \sT \cup \sU' \rceil$ s.t. $Q(Z \mid \sV_Z)=Q(Z \mid \sV'_{\prec Z},\sU')$
%
%$\Leftarrow$
%
%$\forall X \in \sX' \forall Z \in \sZ:Z \dsep (\sC' \setminus \sC_X)_{\prec Z} \mid \lceil \sU' \cup (\sC_X \cup \sX' \cup \sZ)_{\prec Z}\rceil$
%\end{conjecture}
%
%I will now outline the proof sketch.
%
%Step 1: change to graphical criterion.
%It seems like what we actually want is usually a purely graphical condition, 
%rather than a probabalistic one.
%So we can substitute:
%$$Q(Z \mid \sV_Z)=Q(Z\mid \sV_{\prec Z}',\sU') \Leftarrow Z \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sV_Z \mid \lceil \sV_Z \rceil. \qquad (\text{by d-separation})$$
%
%Step 2: choose largest possible subset.
%We should also be able to replace ``there exists a blocking set'' with 
%``the largest available set is blocking'', because if any subset is blocking, then the largest one will be.
%\begin{align*}& \exists \sV_Z \subseteq (\sV'_{\prec Z} \cup \sU') \cap \lceil \sT \cup \sU' \rceil \text{ s.t.\ } Z \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sV_Z \mid \lceil \sV_Z \rceil \\
%&\Longleftrightarrow 
%\sW:=\lceil(\sV'_{\prec Z} \cup \sU') \cap \lceil\sT\cup\sU'\rceil\rceil;
%Z \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sW \mid  \sW. 
%\end{align*}
%
%Step 3: simplify $\sW$.
%We've modified $\fix$ to add to $\sT$ any $Z$ that meets the 
%d-separation condition given predecessors in $\sT$,
%and then to add any determined decision $X \in \lceil \sT \rceil$.
%But whether some $Z$ or $X$ can be added will depend only on predecessors, 
%enabling some simplification.
%
%\begin{align*}
%\sW &=\lceil(\sV'_{\prec Z} \cup \sU') \cap \lceil\sT\cup\sU'\rceil\rceil &&\\
%&=\lceil \sU'\cup (\sV'_{\prec Z} \cap \lceil \sT \cup \sU'\rceil)\rceil && (\sU' \subseteq \lceil\sT\cup\sU\rceil \\
%&=\lceil \sU'\cup ((\sC'\cup\sZ\cup\sX')_{\prec Z} \cap \lceil \sT \cup \sU' \rceil)\rceil &&\text{def of } \sV' \\
%&=\lceil \sU'\cup ((\sC'\cup\sZ\cup\sX')_{\prec Z} \cap (\sT \cup \sU'))\rceil && \text{any $X \in \sX'_{\prec Z}$ in $\lceil\sC_X\rceil$ is also in $\lceil\sC'_{\prec Z}\rceil$} \\
%&= \lceil \sU'\cup ((\sC'\cup\sZ\cup\sX')_{\prec Z} \cap \sT)\rceil && \text{(algebra)}
%\end{align*}

%Step 4: simplify $\hat{\sT}$
%So far, we have:
%\begin{align*}
%&\hat{\sT}=\lceil\sT\rceil \cup \{Z \in \sZ:Z\dsep (\sV'_{\prec Z} \cup \sU') \setminus \sW \mid \sW\} \\
%&\text{where } \sW:=\lceil \sU' \cup ((\sC' \cup \sZ \cup \sX')_{\prec Z} \cap \sT)\rceil \\
%&\text{and }\fix(\sT)=\sT \text{ if } \sT=\hat{\sT} \text{ and } \fix(\hat{\sT}) \text{ otherwise.}
%\end{align*}
%
%This is equivalent to:
%\begin{align*}
%&\hat{\sT}=\lceil\sT_{\prec Z}\rceil \cup \{Z \in \sZ:Z\dsep (\sV'_{\prec Z} \cup \sU') \setminus \sW \mid \sW\} \\
%&\text{where } \sW:=\lceil \sU' \cup ((\sC' \cup \sZ \cup \sX')_{\prec Z} \cap \sT_{\prec Z})\rceil \\
%\end{align*}
%
%because the nodes $\sT$ are intersected with $\sV_{\prec Z}$ anyway.
%This means that we are adding nodes to $\sT$ in increasing order wrt $\prec$.
%%Moreover, $\sT_{\prec Z} \subseteq (\sC' \cup \sZ \cup \sX')_{\prec Z}$, so we can write $\sW=\lceil\sU' \cup (\sC' \cup \sZ \cup \sX')_{\prec Z}\rceil$.
%
%Step 5: simplify $\fix(\sC_X \setminus \sZ) \supseteq \sC_X$.
%Finally, we note that for the result above, it is sufficient that
%$$\forall X \in \sX' \forall Z \in \Pa^\calG_X \cap \sZ:Z \dsep (\sC' \setminus \sC_X)_{\prec Z} \mid \sW.$$
%We prove the result by induction, 
%showing that every $Z$ is d-separated from every $\sV'_{\prec Z} \cup \sU' \setminus \sW$ given $\sW$.
%For the base step, consider for any $X$, the first $Z$, ordered by $\prec$.
%Clearly, it is d-separated from $\sZ_{\prec Z} \setminus \sW=\emptyset$ given $\sW$.
%It is d-separated from $(\sC \setminus C_X)_{\prec Z}$ by assumption, 
%and $C_X \subseteq \T_{\prec Z}$ so it is d-separated from $\sC'_{\prec Z} \setminus \sW$.
%
%
%
%
%Next, we note that any decision will be added to $\sT$ if the latent predecessors $Z_{\prec X}$ have already been added (because Le 1 requires that parents are predecessors).
%So, $\fix(\sC_X \setminus \sZ) \supseteq \sC_X$ can be understood as just 
%checking whether each $Z$ is added to $\sT$ given that its predecessors have 
%already been added.
%Thus, we find that $\forall X \in \sC':\fix(\sC_X \setminus \sZ) \supseteq \sC_X$ is equivalent to
%\begin{align*}
%&&&\forall X \in \sX' \forall Z \in \Pa^\calG_X \cap \sZ:Z \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sW \mid \sW && \\
%&\Longleftrightarrow&& \forall X \in \sX' \forall Z \in \Pa^\calG_X \cap \sZ:Z \dsep (\sC' \setminus \sC_X)_{\prec Z} \mid \sW && (\sV'_{\prec Z} \cup \sU' \setminus \sW=(\sC' \setminus \sC_X)_{\prec Z}) \\
%\end{align*}
%\ryan{Need to flesh out this inductive argument a bit more.}




\begin{lemma}[Simplifying Thm 2]
If 
$\forall X \in \sX' \forall Z \in C_X \cap \sZ:Z \dsep (\sC' \setminus C_X)_{\prec Z} \mid \lceil \sU' \cup (\sV'_{\prec Z} \cap \fix(C_X \setminus \sZ)) \rceil$
and $\sX,\sC',\sZ,\sU'$ satisfy Le 1,
then 
$\sX,\sC',\sZ,\sU',\prec$
satisfy Thm 2
\end{lemma}

\begin{proof}
We prove this result in two steps:
(1) LHS implies that $\forall X \in \sC'$, $\fix'(C_X \setminus \sZ) \supseteq C_X$
where $\fix' (\sT):=\sT$ if $\sT=\bar{\sT}$ and $\fix'(\bar{\sT})$ otherwise,
$\bar{\sT}:=\lceil\sT \rceil \cup \{Z \in \sZ:Z \dsep \sV'_{\prec Z} \setminus \sW \mid \sW \}$,
where 
$\sW:= \sU' \cup (\lceil \sT \rceil \cap \sV'_{\prec Z})$.
(2) for all $\sB$, $\fix(\sB) \supseteq \fix'(\sB)$.

Proof of (1).
We prove the result by induction.
The base step is that for 
any $X \in \sX'$,
for the first $Z \in \sZ$ by $\prec$, 
every $Z' \in \sZ_{\prec Z}$ is in $\fix'(C_X \setminus \sZ)$.
Since $\sZ_{\prec Z}$ is empty, this holds trivially.
The inductive step is that for any $X \in \sX'$,
if every $Z' \in \sZ_{\prec Z}$ is in $\fix'(C_X \setminus \sZ)$
then $Z \in \fix'(C_X \setminus \sZ)$.
%We will prove that at the fixed point $\sT=\fix'(C_X \setminus \sZ)$, 
%every such $Z$ is in $\bar{\sT}$ and therefore in $\fix'(C_X \setminus \sZ)$
%because $Z$ is d-separated from $\sV'_{\prec Z} \setminus \sW$ given $\sW$.
To prove that $Z \in \fix'(C_X \setminus \sZ)$,
we will prove that
$Z \dsep \sV'_{\prec Z} \setminus \sW \mid \sW$, 
at the fixed point of $\bar{\sT}$,
which we show by partitioning $\sA:=\sV'_{\prec Z} \setminus \sW$ into 
$\sA \cap \sZ$, $\sA \cap \sC'$, and $\sA \cap \sX'$.
Every $Z' \in \sA \cap \sZ$ is in $\sZ_{\prec Z} \setminus \sW$.
But by the inductive assumption, $Z' \in \fix'(C_X \setminus \sZ)$, 
so $Z' \in \sW$.
Thus $\sA \cap \sZ = \emptyset$ and $Z \dsep \sA \cap \sZ \setminus \sW \mid \sW$.
In the second partition,
every $C \in \sA \cap \sZ$ is in 
$\sC_{\prec Z} \setminus \sW$ and 
since $\sW \supseteq (C_X)_{\prec Z}$,
$C \in (\sC' \setminus C_X)_{\prec Z}$. 
And $Z \dsep (\sC' \setminus C_X) \mid \sW$
by the assumption in the LHS of the lemma statement.
\ryan{This does not quite match what is on the LHS...}
In the third partition, 
every $X' \in \sX' \cap \sA$ is in $\sX'_{\prec Z} \setminus \sW$.
$X' \not \in \sW$ implies that $X'$ must have a parent $C$ that is not in 
$\fix'(\sC' \setminus C_X)$, 
otherwise every $C \in C_{C_X}$ would be in $\sV'_{\prec Z} \cap \fix'(\sC' \setminus C_X)$ by Le1.3,
and $X' \in \lceil \sV'_{\prec Z} \cap \fix'(C_X \setminus \sZ) \rceil = \sW$.
This $C$ then must not be $C \in C_{X'} \setminus C_X$, because $\fix$ never removes elements.
We know that every path from $Z$ to $C$ is blocked given $\sW$ 
by the LHS of the lemma statement.
And $X$ is not in $\sW$, 
so there cannot be a path from $Z$ to $X$, active given $\sW$ 
(because if there was one, it could be extended with the edge $C \to X$
to form an active path to $C$).
So $Z$ cannot be d-connected given $\sW$ to any $X$ in $\sA \cap \sX'$.
Thus the LHS implies that for each $X \in \sX'$, 
$\fix'(C_X \setminus \sZ) \supseteq C_X$.

Step (2):
Note that $\fix'$ and $\fix$ only differ with respect 
to the conditions for adding an element $Z$.
Whenever an element $Z$ may be added to $\bar{\sT}$ (i.e.\ is in $\bar{\sT}\setminus \sT$), we will prove that it is also in $\hat{\sT}$
(as defined in Thm 2), and hence in $\fix$.
We will infer that $Z \in \hat{\sT}$ from the existence of
$\sV_Z=\lceil \sU' \cup (\lceil \sT \rceil \cap \sV'_{\prec Z}\rceil=\lceil \sW \rceil$.

As required by $\hat{\sT}$, we have that 
$\sV_Z \subseteq \sU' \cup \sV'_{\prec Z}$,
and that 
$\sV_Z \setminus \sU' \subseteq \lceil \sT \rceil$. 
%And
%we have that $Z \dsep (\sV'_{\prec Z} \cup \sU') \setminus \lceil \sV_Z \rceil \mid \lceil \sV_Z \rceil$.
Since $Z \in \bar{\sT}$, we also have
$Z \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sW \mid \sW$.
Since $\sV_Z = \lceil \sW \rceil$, this means
$Z \dsep (\sV'_{\prec Z} \cup \sU') \setminus \sV_Z \mid \lceil \sV_Z \rceil$, and, by the soundness of d-separation, 
$Q(Z \mid \sV_Z) = Q(Z \mid \sV'_{\prec Z},\sU')$.
So $Z$ is also in $\hat{\sT}$.
Since $\fix'$ and $\fix$ are identical in other respects, 
we have $\fix(\sB) \supseteq \fix'(\sB)$ for all $\sB$.

Combining (1-2), we have that if the LHS is true, then for every $X\in \sX'$,
$\fix(C_X \setminus \sZ) \supseteq \fix'(C_X \setminus \sZ) \supseteq C_X$, 
thus Thm 2 is satisfied, proving the result.

\end{proof}
\ryan{I think the first step is an equivalence, but I haven't needed to prove it yet.}





Upshots of this simplification:
\begin{itemize}
    \item We could use this d-connection criterion to add another edge to the ordering graph $\calH$
    \item Then, when we notice a cycle in $\calH$, we would need to consider a second way that there can be an edge $A \to B$ where $B \not \in \Desc^\calG_A$.
\end{itemize}




==> sections/old/z-removed-prelims.tex <==
\section{Preliminaries}

We will make use of the following general result. 
\todo{Instead cite this as the third graphoid axiom, per Robin} \ryan{Where is it proved that the third graphoid axiom holds for DAGs?}
\begin{lemma}[Weak Union Graphoid Axiom] \label{le:move-endpoint-to-condset-preserves-sep}
If $\sA \dsep \sB \mid \sC$
then $\sA \dsep \sB \setminus \sZ \mid \sC \cup \sZ$
for any $\sZ  \subseteq \sB$.
\end{lemma}
\begin{proof}
%See \citep{verma1990causal}
We prove the contrapositive: that $\sA \not \dsep \sB \setminus \sZ \mid \sC \cup \sZ \Rightarrow \sA \not \dsep \sB \mid \sC$.
There must be a path $p$ from $\sA$ to $\sB \setminus \sZ$, active given $\sC \cup \sZ$.
$p$ cannot contain any non-collider in $\sC$.
So if every collider in $p$ is an ancestor of $\sC$, then the result follows.
If instead, there exists a collider in $p$ that is a non-ancestor of $\sC$, then it must be an ancestor of $\sZ$, 
so extend $p$ to the this element of $\sZ$ to obtain a path from $\sA$ to $\sB$, active given $\sC$, proving the result.
\end{proof}

We will also use the following.

\begin{lemma}[maximal conditioning set of ancestors separates] \label{le:max-cond-separates}
    Lemma: let $\mathbf{A} \subseteq Anc(Y)$. 
    If $\exists \mathbf{A}' \subseteq \mathbf{A} : Z \perp Y \mid \mathbf{A'}$, then $Z \perp Y \mid \mathbf{A}$
\end{lemma}
\begin{proof}
Our approach will be to prove that it is impossible to have $Z \not \perp Y \mid \mathbf{A}$ and $Z \perp Y \mid \mathbf{A'}$, 
by way of contradiction.
Suppose that there was a path $p$ from $Z$ to $Y$, active given $\sA$, that was inactive given $\sA'$.
$p$ cannot be blocked by $\sA'$ at a non-collider, since $\sA' \subseteq \sA$.
So consider the collider $V$ nearest $Z$ where $p$ is blocked by $\sA'$.
This collider must be an ancestor of $\sA$ but not an ancestor of $\sA'$.
But in that case, the path $p$ can be extended along any directed path $V \pathto Y$
to obtain a path active given $\sA'$, meaning that $Z \perp Y \mid \mathbf{A'}$, yielding a contradiction.
\end{proof}

\begin{lemma}[Ancestors of closure] \label{le:ancestors-of-closure}
If $V \in \lceil \sV \rceil$ and $A \in \Anc^\calG(V) \setminus \lceil \sV \rceil$ then $A \in \Anc^\calG(\sV)$
\end{lemma}
\begin{proof}
We will prove the contrapositive CP: that if $A \not \in \Anc^\calG(\sV)$
then 
$V \not \in \lceil \sV \rceil$ or $A \not \in \Anc^\calG(V) \setminus \lceil \sV \rceil$.
In the case where $A \not \in \Anc^\calG(\sV)$
and $A \not \in \Anc^\calG(V) \setminus \lceil \sV \rceil$,
(CP) is clearly true.
In the remaining case, $A \not \in \Anc^\calG (\sV)$
and 
$A \in \Anc^\calG(V) \setminus \lceil \sV \rceil$, and
we will prove that $V \not \in \lceil \sV \rceil$.
Choose any path $p:A = N^1 \to N^2 \to ... \to N^n = V$.
Then, every $N^i$ is not in $\sV$ by assumption.
Moreover, $A=N^1 \not \in \lceil \sV \rceil$,
and $N^{i-1} \not \in \lceil \sV \rceil \implies N^i \not \in \lceil \sV \rceil$
by the definition of $\lceil \cdot \rceil$.
So by induction, $V=N^n \not \in \lceil \sV \rceil$, 
and (CP) is true again, proving the result.
\end{proof}

The problem with condition (1) of the lemma above is that it is stated in terms of $\sX'$ and $\sC'$, which are free parameters that the theorem is quantified over, 
whereas what we want is to know what paths must be present in terms of the decision $\sX(\calS)$ and contexts $C_{\sX(\calS)}$ of the graph.
In order to obtain the simpler expression for this condition, that is used in the main paper, we use the following result.
The logic is that we can fix $\sX'$ and $\sC'$ by selecting the largest possible set of decisions and contexts to obtain a simpler expression.

\begin{lemma} \label{le:cond1.1-unsatisfiable}
Let $\calS$ be a scope with decision $X$ and context $Z \in C_X$.
If every $\sX',\sC'$ such that $X \in \sX' \subseteq \sX(\calS) \setminus Z,\sC' \subseteq C_{\sX'} \setminus (\sX' \cup Z)$
has $(Y \not \dsep_{\calG_\calS} \Pi_X) \mid \lceil \sX' \cup \sC' \rceil$, 
%If Cond. 1.1 is unsatisfiable for $Z \! \to \!X \in \!\sX(\calS)$ in $\calG_\calS$, 
then $(Z \!\not \dsep_{\calG_\calS} Y)\! \mid {\condset{\set{Z}}}$.
\end{lemma}
\begin{proof}
%We prove the result by contrapositive.
%If $Z \dsep Y \mid \condset{Z}$, 
%then choose $\sX'=\sX(\calS)  \setminus Z,\sZ=Z,\sC'=\sC_{\sX(\calS) \setminus Z}\setminus Z$, and Condition 1.1 is satisfied
%for $Z \to X$. The result follows.
%This proves that $Z \not \dsep Y \mid \condset{Z}$

%We prove the result by contrapositive.
It follows from assumption that $(Y \dsep_{\calG_\calS} \Pi_X) \mid \lceil \sX' \cup \sC' \rceil$ for
%$\sZ=\set{Z}$ and 
$\sX'=\sX(\calS)\setminus Z$ and $\sC' =\sC_{\sX'} \setminus (\sX' \cup Z)$. 
We can then express the conditioning set as:
\begin{align*}
   \sX' \cup \sC'  &= (\sX(\calS)\setminus Z) \cup (\sC_{\sX(\calS)\setminus Z} \setminus ((\sX(\calS)\setminus Z) \cup Z))\\ 
   &= (\sX(\calS)\setminus Z) \cup (\sC_{\sX(\calS)\setminus Z} \setminus (\sX(\calS) \cup Z)) \\
%   &= (\sX(\calS)\setminus Z) \cup ((\sC_{\sX(\calS)\setminus Z} \setminus \sX(\calS)) \setminus Z)) \\
   &= (\sX(\calS) \cup \sC_{\sX(\calS)\setminus Z}) \setminus Z.
\end{align*}
This means that there is an active path from $\Pi_X$ to $Y$ given $(\sX(\calS) \cup \sC_{\sX(\calS)\setminus Z}) \setminus Z$.
Note that any d-connecting path from $\Pi_X$ to $Y$ must start with $\Pi_X \to X \gets Z$ because $X$ is in the conditioning set and the parents of $X$ other than $Z$ are all blocked. 
So we can truncate this path as $Z \upathto Y$, which is active given $(\sX(\calS) \cup \sC_{\sX(\calS)\setminus Z}) \setminus Z$, 
which proves the result.
\end{proof}

==> toward-complete-authorship.tex <==
\begingroup
\baselineskip=18pt plus1pt
\setlength{\parindent}{0pt}
\setlength{\parskip}{0.5em}
\section*{Statement of Authorship}\thispagestyle{empty}

\textbf{Title of Paper}: Toward a Complete Criterion for Value of
Information in Insoluble Decision Problems

\textbf{Publication Status:} Unpublished work written in a journal paper style, in review

\textbf{Publication Details:} 
Ryan Carey, Sanghack Lee, and Robin J. Evans. Toward a Complete Criterion for Value of Information in Insoluble Decision Problems, in review.

\textbf{Student name:} Ryan Carey

\textbf{Contribution to the paper:}
Ryan led the project, while Robin and Sanghack were active supervisors.

Ryan devised the proof strategies, and regularly discussed progress with Sanghack and Robin, who provided extensive suggestions and comments throughout the project.

\vspace{0\baselineskip}

Signature:

\vspace{1\baselineskip}
\rule{7cm}{0.4pt}

%\vspace{\baselineskip}
Date:

\vspace{0.7\baselineskip}

\emph{The candidate made a substantial contribution to the publication, and the description above is accurate.}

\textbf{Co-author Name:} Sanghack Lee

Signature:

\vspace{0.7\baselineskip}
\rule{7cm}{0.4pt}

Date:

%\emph{The candidate made a substantial contribution to the publication, and the description above is accurate.}

\textbf{Co-author/Supervisor Name:} Robin J. Evans

Signature:

\vspace{0.7\baselineskip}
\rule{7cm}{0.4pt}

Date:

\endgroup



